Spectroscopy of The Largest Ever Gamma-ray Selected BL Lac Sample

We report on spectroscopic observations covering most of the 475 BL Lacs in the 2nd Fermi LAT catalog of AGN. Including archival measurements (correcting several erroneous literature values) we now have spectroscopic redshifts for 44% of the BL Lacs. We establish firm lower redshift limits via intervening absorption systems and statistical lower limits via searches for host galaxies for an additional 51% of the sample leaving only 5% of the BL Lacs unconstrained. The new redshifts raise the median spectroscopic z from 0.23 to 0.33 and include redshifts as large as z=2.471. Spectroscopic redshift minima from intervening absorbers have ~ z= 0.70, showing a substantial fraction at large z and arguing against strong negative evolution. We find that detected BL Lac hosts are bright ellipticals with black hole masses M_\bullet ~ 10^{8.5-9}, substantially larger than the mean of optical AGN and LAT Flat Spectrum Radio Quasar samples. A slow increase in M_\bullet with z may be due to selection bias. We find that the power-law dominance of the optical spectrum extends to extreme values, but this does not strongly correlate with the gamma-ray properties, suggesting that strong beaming is the primary cause of the range in continuum dominance.

==> table3.tex <==
2FGL J0000.9$-$0748 & 0.325017 & $-$7.774111 & J0001$-$0746 & 1.55$\pm$0.11 & $-$1.399$\pm$0.003 & ... & ... & . & ... & 0.33 & 0.50 & 1.84 & BLL & IBL & P200 & 55064\\
2FGL J0007.8+4713 & 1.999862 & 47.202135 & J0007+4712 & 1.32$\pm$0.14 & $-$1.695$\pm$0.071 & ... & 2.1: & S & 1.659 & 0.26 & 0.36 & 2.69 & BLL & LBL & P200 & 55743\\
2FGL J0009.0+0632 & 2.267006 & 6.472664 & J0009+0628 & 1.38$\pm$0.11 & $-$1.410$\pm$0.007 & ... & ... & . & ... & 0.58 & 0.76 & 1.65 & BLL & LBL & WMKO & 55040\\
2FGL J0009.1+5030 & 2.344750 & 50.508005 & J0009+5030 & 1.51$\pm$0.11 & $-$0.776$\pm$0.010 & ... & ... & . & ... & 0.79 & 0.79 & 1.64 & BLL & . & WMKO & 55475\\
2FGL J0012.9$-$3954 & 3.249804 & $-$39.907184 & J0012$-$3954 & 1.01$\pm$0.11 & $-$1.248$\pm$0.032 & ... & ... & . & ... & 0.52 & 0.64 & 2.52 & BLL & . & VLT & 54362\\
2FGL J0013.8+1907 & 3.485099 & 19.178246 & J0013+1910 & 0.61$\pm$0.11 & $-$2.250$\pm$0.076 & ... & 0.477 & B & ... & 0.41 & 0.54 & 2.17 & BLL & . & WMKO & 54470\\
2FGL J0018.5+2945 & 4.615626 & 29.791743 & J0018+2947 & 1.13$\pm$0.11 & $-$0.701$\pm$0.181 & ... & ... & . & ... & 0.89 & 0.94 & 1.71 & BLL & HBL & WMKO & 55547\\
2FGL J0018.8$-$8154 & 4.841042 & $-$81.880833 & J0019$-$8152 & 1.73$\pm$0.12 & $-$0.975$\pm$0.045 & ... & ... & . & ... & 0.24 & 0.34 & 2.32 & BLL & HBL & NTT & 55778\\
2FGL J0021.6$-$2551 & 5.385517 & $-$25.846999 & J0021$-$2550 & 1.63$\pm$0.11 & $-$0.689$\pm$0.005 & ... & ... & . & 0.564 & 0.57 & 0.58 & 1.63 & BLL & IBL & WMKO & 55476\\
2FGL J0022.2$-$1853 & 5.538158 & $-$18.892486 & J0022$-$1853 & 1.94$\pm$0.11 & $-$1.061$\pm$0.069 & ... & ... & . & 0.774 & 0.13 & 0.15 & 1.64 & BLL & HBL & WMKO & 55476\\
2FGL J0022.5+0607 & 5.635264 & 6.134573 & J0022+0608 & 1.86$\pm$0.11 & $-$1.560$\pm$0.009 & ... & ... & . & ... & 0.29 & 0.42 & 1.63 & BLL & LBL & WMKO & 55060\\
2FGL J0029.2$-$7043 & 7.170792 & $-$70.754694 & J0028$-$7045 & 1.38$\pm$0.11 & $-$1.139$\pm$0.011 & ... & ... & . & 0.966 & 0.54 & 0.58 & 1.95 & BLL & . & VLT & 55056\\
2FGL J0033.5$-$1921 & 8.393060 & $-$19.359393 & J0033$-$1921 & 1.94$\pm$0.12 & $-$0.852$\pm$0.053 & ... & ... & . & ... & 0.29 & 0.37 & 1.77 & BLL & HBL & P200 & 55567\\
2FGL J0035.2+1515 & 8.810913 & 15.250758 & J0035+1515 & 1.93$\pm$0.11 & $-$0.895$\pm$0.003 & ... & ... & . & ... & 0.48 & 0.48 & 1.65 & BLL & HBL & WMKO & 55357\\
2FGL J0037.8+1238 & 9.461902 & 12.638514 & J0037+1238 & 2$\pm$0.11 & $-$1.163$\pm$0.010 & $-$22.4$\pm$0.10 & 0.089 & G & ... & 0.09 & 0.09 & 1.76 & BLL & HBL & WMKO & 55357\\
2FGL J0038.1+0015 & 9.535594 & 0.226673 & J0038+0013 & 0.86$\pm$0.11 & $-$1.649$\pm$0.015 & ... & ... & . & ... & 0.48 & 0.64 & 2.23 & BLL & . & SDSS & 52944\\
2FGL J0045.5+1218 & 11.430701 & 12.286122 & J0045+1217 & 1.83$\pm$0.12 & $-$1.249$\pm$0.131 & ... & ... & . & ... & 0.25 & 0.37 & 1.62 & BLL & HBL & P200 & 55567\\
2FGL J0045.3+2127 & 11.330296 & 21.461857 & J0045+2127 & 1.89$\pm$0.11 & $-$0.725$\pm$0.013 & ... & ... & . & ... & 0.42 & 0.42 & 1.78 & BLL & HBL & WMKO & 55040\\
2FGL J0047.2+5657 & 11.752236 & 56.961705 & J0047+5657 & 1.13$\pm$0.13 & $-$1.155$\pm$0.389 & ... & ... & . & ... & 0.64 & 0.77 & 1.97 & BLL & . & WMKO & 55358\\
2FGL J0050.2+0234 & 12.430146 & 2.617458 & J0049+0237 & 1.26$\pm$0.11 & $-$1.177$\pm$0.021 & ... & 1.474 & B & 1.474 & 0.72 & 0.88 & 1.65 & BLL & . & WMKO & 55476\\
2FGL J0050.6$-$0929 & 12.671950 & $-$9.485096 & J0050$-$0929 & 1.38$\pm$0.12 & $-$1.276$\pm$0.276 & ... & 0.635 & N & ... & 0.32 & 0.53 & 2.18 & BLL & IBL & WMKO & 55358\\
2FGL J0055.0$-$2454 & 13.694860 & $-$24.924764 & J0054$-$2455 & 1.87$\pm$0.11 & $-$0.290$\pm$0.023 & ... & ... & . & ... & 0.61 & 0.61 & 1.63 & BLL & HBL & WMKO & 55476\\
2FGL J0056.8$-$2111 & 14.134439 & $-$21.285629 & J0056$-$2117 & 1.64$\pm$0.11 & $-$0.754$\pm$0.032 & ... & ... & . & 0.873 & 0.67 & 0.83 & 1.62 & BLL & IBL & WMKO & 55476\\
2FGL J0057.9$-$3236 & 14.509433 & $-$32.571785 & J0058$-$3234 & 1.37$\pm$0.11 & $-$0.775$\pm$0.071 & ... & ... & . & ... & 0.58 & 0.77 & 1.93 & BLL & LBL & VLT & 55055\\
2FGL J0059.2$-$0151 & 14.820240 & $-$1.838233 & J0059$-$0150 & 1.12$\pm$0.12 & $-$1.394$\pm$0.106 & $-$22.57$\pm$0.17 & 0.144 & G & ... & 0.14 & 0.14 & 2.76 & BLL & HBL & NTT & 55778\\
2FGL J0100.2+0746 & 15.086698 & 7.764155 & J0100+0745 & -0.27$\pm$0.24 & $-$5.689$\pm$0.740 & ... & ... & . & ... & 0.66 & 0.76 & 4.01 & BLL & . & WMKO & 55040\\
2FGL J0105.3+3930 & 16.288374 & 39.470855 & J0105+3928 & 0.86$\pm$0.13 & $-$1.351$\pm$0.114 & $-$22.37$\pm$0.20 & 0.440 & G & ... & 0.44 & 0.59 & 2.68 & BLL & . & HET & 55422\\
2FGL J0109.0+1817 & 17.284165 & 18.268477 & J0109+1816 & 1.92$\pm$0.12 & $-$1.336$\pm$0.030 & $-$23.59$\pm$0.32 & 0.443 & G & ... & 0.33 & 0.44 & 2.48 & BLL & HBL & HET & 55479\\
2FGL J0110.3+6805 & 17.552543 & 68.094833 & J0110+6805 & 2.54$\pm$0.13 & $-$0.759$\pm$0.209 & ... & ... & . & 0.327 & 0.11 & 0.12 & 1.78 & BLL & IBL & WMKO & 55475\\
2FGL J0114.7+1326 & 18.719670 & 13.426800 & J0114+1325 & 1.8$\pm$0.11 & $-$0.543$\pm$0.008 & ... & ... & . & ... & 0.61 & 0.71 & 1.63 & BLL & . & WMKO & 55476\\
2FGL J0115.4+0358 & 18.918771 & 3.945195 & J0115+0356 & 1.72$\pm$0.11 & $-$0.569$\pm$0.071 & ... & ... & . & 0.140 & 0.67 & 0.80 & 1.62 & BLL & . & WMKO & 55476\\
2FGL J0115.7+2518 & 18.942122 & 25.331770 & J0115+2519 & 1.93$\pm$0.11 & $-$0.739$\pm$0.003 & ... & ... & . & 0.268 & 0.37 & 0.37 & 1.63 & BLL & HBL & WMKO & 55061\\
2FGL J0120.4$-$2700 & 20.132100 & $-$27.023566 & J0120$-$2701 & 2.03$\pm$0.11 & $-$1.385$\pm$0.001 & ... & ... & . & 0.558 & 0.36 & 0.39 & 1.76 & BLL & LBL & P200 & 55423\\
2FGL J0124.5$-$0621 & 21.210332 & $-$6.417219 & J0124$-$0625 & 1.26$\pm$0.12 & $-$1.621$\pm$0.013 & ... & 2.117 & S & 2.117 & 0.48 & 0.50 & 2.24 & BLL & . & WMKO & 55061\\
2FGL J0134.4+2636 & 23.616643 & 26.645097 & J0134+2638 & 0.24$\pm$0.16 & $-$0.460$\pm$0.444 & ... & ... & . & ... & 0.41 & 0.46 & 3.88 & UNK & HBL & HET & 55422\\
2FGL J0136.5+3905 & 24.135135 & 39.099797 & J0136+3905 & 2.31$\pm$0.11 & $-$0.323$\pm$0.008 & ... & ... & . & ... & 0.75 & 0.88 & 1.65 & BLL & HBL & WMKO & 55475\\
2FGL J0141.5$-$0928 & 25.357507 & $-$9.478993 & J0141$-$0928 & 1.9$\pm$0.11 & $-$1.331$\pm$0.010 & $-$24.24$\pm$0.28 & 0.735 & G & 0.501 & 0.45 & 0.48 & 2.17 & BLL & IBL & SDSS & 52174\\
2FGL J0144.6+2704 & 26.139726 & 27.084218 & J0144+2705 & 1.66$\pm$0.14 & $-$4.272$\pm$0.319 & ... & ... & . & 0.708 & 0.31 & 0.40 & 1.66 & BLL & LBL & WMKO & 55060\\
2FGL J0148.6+0127 & 27.140702 & 1.483598 & J0148+0129 & 0.93$\pm$0.12 & $-$1.025$\pm$0.255 & ... & 0.940 & N & ... & 0.83 & 0.90 & 1.68 & BLL & . & WMKO & 55476\\
2FGL J0153.9+0823 & 28.511543 & 8.397419 & J0154+0823 & 2.1$\pm$0.11 & $-$0.661$\pm$0.004 & ... & 0.681 & N & 0.341 & 0.48 & 0.63 & 1.64 & BLL & IBL & WMKO & 55476\\
2FGL J0154.9+4434 & 28.727484 & 44.560169 & J0154+4433 & 1.74$\pm$0.11 & $-$0.749$\pm$0.171 & ... & ... & . & 0.386 & 0.67 & 0.77 & 1.63 & BLL & . & WMKO & 55475\\
2FGL J0158.3$-$3931 & 29.658856 & $-$39.534427 & J0158$-$3932 & 1.28$\pm$0.11 & $-$0.947$\pm$0.038 & ... & ... & . & ... & 0.80 & 0.83 & 2.15 & BLL & LBL & VLT & 55191\\
2FGL J0159.6$-$2741 & 29.930696 & $-$27.677319 & J0159$-$2740 & 1.48$\pm$0.11 & $-$1.240$\pm$0.003 & ... & ... & . & 0.578 & 0.54 & 0.63 & 1.78 & BLL & IBL & P200 & 55152\\
2FGL J0159.5+1046 & 29.893369 & 10.784943 & J0159+1047 & 1.74$\pm$0.11 & $-$1.048$\pm$0.011 & $-$22.06$\pm$0.16 & 0.195 & G & ... & 0.20 & 0.56 & 1.76 & BLL & HBL & P200 & 55152\\
2FGL J0204.0+3045 & 30.934127 & 30.710634 & J0203+3042 & 2.2$\pm$0.11 & $-$1.495$\pm$0.006 & ... & 0.761 & B & ... & 0.23 & 0.30 & 2.72 & BLL & . & HET & 55483\\
2FGL J0203.6+7235 & 30.888386 & 72.548336 & J0203+7232 & 1.83$\pm$0.11 & $-$1.237$\pm$0.040 & ... & ... & . & ... & 0.37 & 0.46 & 2.47 & BLL & LBL & HET & 55102\\
2FGL J0207.9$-$6832 & 31.963542 & $-$68.631836 & J0207$-$6837 & 0.97$\pm$0.11 & $-$1.537$\pm$0.077 & ... & ... & . & 0.680 & 0.43 & 0.50 & 2.64 & BLL & . & NTT & 55776\\
2FGL J0209.5$-$5229 & 32.339833 & $-$52.489778 & J0209$-$5229 & 1.46$\pm$0.11 & $-$0.672$\pm$0.021 & ... & ... & . & ... & 0.31 & 0.39 & 2.18 & BLL & HBL & NTT & 55205\\
2FGL J0211.2+1050 & 32.805000 & 10.859538 & J0211+1051 & 3.03$\pm$0.11 & $-$0.812$\pm$0.001 & ... & ... & . & ... & 0.12 & 0.22 & 1.67 & BLL & IBL & WMKO & 55476\\
2FGL J0213.1+2245 & 33.219930 & 22.748599 & J0212+2244 & 3.05$\pm$0.12 & $-$1.202$\pm$0.072 & ... & 0.459: & S & ... & 0.07 & 0.11 & 2.66 & BLL & HBL & HET & 55124\\
2FGL J0216.9$-$6630 & 34.211875 & $-$66.612000 & J0216$-$6636 & 1.57$\pm$0.11 & $-$0.466$\pm$0.100 & ... & ... & . & 0.673 & 0.52 & 0.61 & 1.94 & BLL & HBL & VLT & 55056\\
2FGL J0217.4+0836 & 34.321278 & 8.617522 & J0217+0837 & 2.02$\pm$0.11 & $-$1.559$\pm$0.033 & $-$21.77$\pm$0.12 & 0.085 & G & ... & 0.27 & 0.30 & 2.12 & BLL & IBL & P200 & 55424\\
2FGL J0222.6+4302 & 35.664530 & 43.035647 & J0222+4302 & 3.05$\pm$0.11 & $-$1.105$\pm$... & ... & ... & . & ... & 0.12 & 0.30 & 1.67 & BLL & IBL & WMKO & 55475\\
2FGL J0238.6$-$3117 & 39.635142 & $-$31.283030 & J0238$-$3116 & 2.11$\pm$0.11 & $-$0.224$\pm$0.003 & $-$22.63$\pm$0.11 & 0.232 & G & ... & 0.23 & 0.23 & 1.63 & BLL & HBL & WMKO & 55476\\
2FGL J0242.9+7118 & 40.878267 & 71.338201 & J0243+7120 & 1.62$\pm$0.16 & $-$0.383$\pm$0.911 & ... & ... & . & 0.998 & 0.28 & 0.32 & 2.26 & BLL & LBL & WMKO & 55547\\
2FGL J0250.6+1713 & 42.572814 & 17.136070 & J0250+1708 & 0.85$\pm$0.19 & $-$1.650$\pm$0.077 & ... & 0.612 & N & ... & 0.41 & 0.41 & 3.81 & BLL & . & HET & 55213\\
2FGL J0257.9+2025 & 44.530362 & 20.500342 & J0258+2030 & 2.44$\pm$0.13 & $-$0.718$\pm$0.290 & ... & ... & . & ... & 0.09 & 0.09 & 2.76 & BLL & HBL & WMKO & 55061\\
2FGL J0303.5+4713 & 45.897017 & 47.271167 & J0303+4716 & 2.34$\pm$0.11 & $-$1.397$\pm$0.001 & ... & ... & . & ... & 0.37 & 0.46 & 1.63 & BLL & LBL & WMKO & 55475\\
2FGL J0314.2$-$5106 & 48.606917 & $-$51.075556 & J0314$-$5104 & 1.06$\pm$0.11 & $-$0.899$\pm$0.058 & ... & ... & . & ... & 0.76 & 0.93 & 1.95 & BLL & . & VLT & 55056\\
2FGL J0316.1+0904 & 49.052976 & 9.078863 & J0316+0904 & 2.88$\pm$0.11 & $-$0.865$\pm$0.002 & ... & ... & . & ... & 0.12 & 0.23 & 1.66 & BLL & HBL & WMKO & 55061\\
2FGL J0316.6+4119 & 49.178961 & 41.324602 & J0316+4119 & 2.09$\pm$0.12 & $-$1.993$\pm$0.080 & $-$22.03$\pm$0.13 & 0.019 & G & ... & 0.02 & 0.10 & 2.21 & BLL & . & SDSS & 52976\\
2FGL J0323.6$-$0108 & 50.931339 & $-$1.196185 & J0323$-$0111 & 1.79$\pm$0.11 & $-$0.908$\pm$0.359 & ... & ... & . & ... & 0.44 & 0.45 & 2.17 & BLL & HBL & SDSS & 52199\\
2FGL J0333.7+2918 & 53.454248 & 29.275409 & J0333+2916 & 2.58$\pm$0.12 & $-$0.213$\pm$0.049 & ... & ... & . & ... & 0.14 & 0.21 & 2.61 & BLL & IBL & HET & 55213\\
2FGL J0334.3+6538 & 53.486319 & 65.615618 & J0333+6536 & 1.79$\pm$0.11 & $-$1.244$\pm$0.062 & ... & ... & . & ... & 0.30 & 0.37 & 2.41 & BLL & IBL & WMKO & 55475\\
2FGL J0334.3$-$3728 & 53.564244 & $-$37.428825 & J0334$-$3725 & 2.54$\pm$0.11 & $-$0.830$\pm$0.001 & ... & ... & . & ... & 0.39 & 0.43 & 1.92 & BLL & LBL & VLT & 55191\\
2FGL J0334.2$-$4008 & 53.556500 & $-$40.140833 & J0334$-$4008 & 0.73$\pm$0.11 & $-$1.463$\pm$0.075 & ... & 1.357 & B & 1.207 & 0.72 & 0.87 & 2.05 & BLL & IBL & VLT & 55191\\
2FGL J0357.0$-$4950 & 59.250500 & $-$49.930750 & J0357$-$4955 & 2.02$\pm$0.11 & $-$0.936$\pm$0.057 & ... & 0.643 & N & ... & 0.47 & 0.64 & 1.92 & BLL & IBL & VLT & 55191\\
2FGL J0402.0$-$2616 & 60.503279 & $-$26.260839 & J0402$-$2615 & 1.22$\pm$0.12 & $-$0.808$\pm$0.021 & ... & ... & . & 1.485 & 0.43 & 0.59 & 1.72 & BLL & LBL & WMKO & 55476\\
2FGL J0423.8+4149 & 65.983245 & 41.834123 & J0423+4150 & 2.03$\pm$0.11 & $-$1.413$\pm$0.039 & ... & ... & . & ... & 0.13 & 0.17 & 2.80 & BLL & . & WMKO & 55060\\
2FGL J0424.7+0034 & 66.195174 & 0.601838 & J0424+0036 & 2.42$\pm$0.11 & $-$0.755$\pm$0.002 & $-$22.7$\pm$0.16 & 0.268 & G & ... & 0.27 & 0.27 & 2.31 & BLL & LBL & WMKO & 55476\\
2FGL J0424.3$-$5332 & 66.266917 & $-$53.532917 & J0425$-$5331 & 1.47$\pm$0.11 & $-$1.220$\pm$0.052 & ... & ... & . & ... & 0.38 & 0.45 & 1.62 & BLL & IBL & NTT & 55778\\
2FGL J0430.4$-$2507 & 67.566900 & $-$25.127422 & J0430$-$2507 & 1.4$\pm$0.11 & $-$0.910$\pm$0.013 & $-$22.37$\pm$0.16 & 0.516 & G & ... & 0.51 & 0.72 & 1.98 & BLL & LBL & VLT & 55191\\
2FGL J0433.5+2905 & 68.407520 & 29.098967 & J0433+2905 & 1.66$\pm$0.13 & $-$1.092$\pm$0.220 & ... & ... & . & ... & 0.56 & 0.62 & 1.79 & BLL & LBL & WMKO & 55475\\
2FGL J0434.1$-$2014 & 68.533022 & $-$20.254802 & J0434$-$2015 & 1.25$\pm$0.11 & $-$1.310$\pm$0.047 & ... & 0.928 & B & ... & 0.65 & 0.79 & 2.43 & BLL & . & VLT & 55191\\
2FGL J0435.1$-$2341 & 68.620756 & $-$23.701666 & J0434$-$2342 & 0.8$\pm$0.11 & $-$1.021$\pm$0.024 & ... & ... & . & ... & 0.55 & 0.55 & 3.35 & UNK & . & NTT & 55778\\
2FGL J0438.8$-$4521 & 69.753708 & $-$45.373333 & J0439$-$4522 & 0.18$\pm$0.12 & $-$1.493$\pm$0.136 & ... & 2.017: & B & 0.979 & 0.77 & 0.83 & 2.72 & BLL & LBL & VLT & 54362\\
2FGL J0440.9+2749 & 70.209785 & 27.846542 & J0440+2750 & 2.04$\pm$0.11 & $-$0.572$\pm$0.009 & ... & ... & . & ... & 0.23 & 0.28 & 2.00 & BLL & . & P200 & 55152\\
2FGL J0448.5$-$1633 & 72.156847 & $-$16.545259 & J0448$-$1632 & 1.67$\pm$0.11 & $-$0.206$\pm$0.049 & ... & ... & . & ... & 0.77 & 0.81 & 1.63 & BLL & HBL & WMKO & 55476\\
2FGL J0505.4+0419 & 76.395087 & 4.265184 & J0505+0415 & 1.48$\pm$0.11 & $-$0.793$\pm$0.005 & ... & ... & . & ... & 0.32 & 0.34 & 2.31 & BLL & HBL & NTT & 55207\\
2FGL J0505.9+6116 & 76.494773 & 61.226681 & J0505+6113 & 2.15$\pm$0.13 & 0.291$\pm$0.034 & ... & ... & . & ... & 0.23 & 0.28 & 2.64 & BLL & HBL & HET & 55178\\
2FGL J0508.0+6737 & 76.982726 & 67.623296 & J0507+6737 & 2.29$\pm$0.11 & $-$0.521$\pm$0.019 & $-$23.56$\pm$0.21 & 0.340 & G & ... & 0.23 & 0.30 & 2.51 & BLL & HBL & HET & 55471\\
2FGL J0509.4+0542 & 77.358222 & 5.693213 & J0509+0541 & 2.75$\pm$0.11 & $-$0.480$\pm$0.034 & ... & ... & . & ... & 0.21 & 0.32 & 1.66 & BLL & IBL & WMKO & 55476\\
2FGL J0509.9+1802 & 77.428722 & 18.108148 & J0509+1806 & 0.08$\pm$0.18 & $-$0.387$\pm$0.476 & ... & ... & . & ... & 0.63 & 0.64 & 6.17 & UNK & . & HET & 55265\\
2FGL J0515.9+1528 & 78.947558 & 15.454671 & J0515+1527 & 2.01$\pm$0.11 & $-$0.436$\pm$0.014 & ... & ... & . & ... & 0.36 & 0.36 & 1.93 & BLL & . & WMKO & 55476\\
2FGL J0516.8$-$6207 & 79.186208 & $-$62.118000 & J0516$-$6207 & 1.74$\pm$0.11 & $-$0.933$\pm$0.016 & ... & 1.300 & B & ... & 0.59 & 0.67 & 1.87 & BLL & IBL & VLT & 55191\\
2FGL J0515.5+7355 & 79.129708 & 73.852423 & J0516+7351 & 1.22$\pm$0.11 & $-$1.585$\pm$0.114 & ... & 0.251 & N & ... & 0.45 & 0.50 & 1.67 & BLL & HBL & P200 & 55152\\
2FGL J0521.7+2113 & 80.441669 & 21.214292 & J0521+2112 & 2.73$\pm$0.11 & $-$0.801$\pm$0.001 & ... & 0.108 & N & ... & 0.11 & 0.12 & 1.70 & BLL & IBL & WMKO & 55475\\
2FGL J0532.5$-$7223 & 83.434292 & $-$72.273028 & J0533$-$7216 & 0.73$\pm$0.14 & 0.285$\pm$0.247 & ... & ... & . & 0.738 & 0.31 & 0.44 & 4.38 & BLL & . & NTT & 55776\\
2FGL J0536.2$-$3348 & 84.121299 & $-$33.717370 & J0536$-$3343 & 1.16$\pm$0.11 & $-$0.222$\pm$0.036 & ... & ... & . & ... & 0.43 & 0.54 & 2.17 & BLL & HBL & NTT & 55205\\
2FGL J0538.5$-$3909 & 84.543078 & $-$39.145604 & J0538$-$3908 & 1.18$\pm$0.11 & $-$1.412$\pm$0.018 & ... & ... & . & ... & 0.32 & 0.32 & 3.15 & UNK & HBL & NTT & 55778\\
2FGL J0540.4+5822 & 85.124905 & 58.394275 & J0540+5823 & 1.74$\pm$0.13 & $-$0.562$\pm$0.107 & ... & ... & . & ... & 0.24 & 0.28 & 2.13 & BLL & HBL & P200 & 55567\\
2FGL J0543.9$-$5532 & 85.986667 & $-$55.534417 & J0543$-$5532 & 1.33$\pm$0.11 & $-$0.610$\pm$0.007 & ... & ... & . & ... & 0.27 & 0.38 & 2.57 & BLL & HBL & NTT & 55207\\
2FGL J0558.7$-$7501 & 89.692375 & $-$74.985083 & J0558$-$7459 & 1.44$\pm$0.12 & $-$1.368$\pm$0.013 & ... & ... & . & 0.475 & 0.29 & 0.38 & 2.20 & BLL & . & NTT & 55206\\
2FGL J0607.4+4739 & 91.846761 & 47.663085 & J0607+4739 & 2.25$\pm$0.11 & $-$1.326$\pm$0.011 & ... & ... & . & ... & 0.22 & 0.28 & 1.70 & BLL & IBL & WMKO & 55061\\
2FGL J0609.4$-$0248 & 92.312571 & $-$2.798412 & J0609$-$0247 & 1.97$\pm$0.11 & $-$0.757$\pm$0.007 & ... & ... & . & ... & 0.37 & 0.37 & 2.48 & BLL & HBL & HET & 55511\\
2FGL J0609.6$-$1847 & 92.574676 & $-$18.794430 & J0610$-$1847 & 1.23$\pm$0.11 & $-$1.510$\pm$0.007 & ... & ... & . & 1.473 & 0.42 & 0.54 & 2.29 & BLL & LBL & P200 & 54450\\
2FGL J0612.8+4122 & 93.213299 & 41.377018 & J0612+4122 & 1.8$\pm$0.11 & $-$1.035$\pm$0.020 & ... & ... & . & 1.108 & 0.27 & 0.35 & 1.80 & BLL & . & P200 & 55152\\
2FGL J0617.6$-$1716 & 94.390321 & $-$17.256166 & J0617$-$1715 & 1.12$\pm$0.18 & $-$0.081$\pm$0.585 & $-$22.9$\pm$0.32 & 0.098 & G & ... & 0.09 & 0.10 & 1.75 & BLL & LBL & NTT & 55207\\
2FGL J0616.9+5701 & 94.320538 & 57.021260 & J0617+5701 & 1.86$\pm$0.11 & $-$1.170$\pm$0.002 & ... & ... & . & 0.796 & 0.46 & 0.51 & 3.94 & BLL & IBL & P200 & 55152\\
2FGL J0621.9+3750 & 95.490088 & 37.849063 & J0621+3750 & 0.85$\pm$0.17 & $-$1.945$\pm$2.224 & ... & ... & . & ... & 0.33 & 0.41 & 2.85 & UNK & . & WMKO & 55061\\
2FGL J0625.2+4441 & 96.326131 & 44.667127 & J0625+4440 & 1.5$\pm$0.11 & $-$1.442$\pm$0.102 & ... & ... & . & 0.311 & 0.74 & 0.75 & 1.64 & BLL & . & WMKO & 55475\\
2FGL J0628.9$-$6246 & 97.238833 & $-$62.812389 & J0628$-$6248 & 0.71$\pm$0.12 & $-$1.094$\pm$0.388 & ... & ... & . & ... & 0.69 & 0.77 & 2.91 & BLL & . & VLT & 54101\\
2FGL J0629.3$-$2001 & 97.349094 & $-$19.988810 & J0629$-$1959 & 1.29$\pm$0.12 & $-$0.990$\pm$0.099 & ... & 1.724: & S & 1.724 & 0.41 & 0.43 & 1.90 & BLL & . & WMKO & 55476\\
2FGL J0630.9$-$2406 & 97.747897 & $-$24.112628 & J0630$-$2406 & 2.33$\pm$0.11 & $-$0.749$\pm$0.094 & ... & ... & . & 1.239 & 0.21 & 0.29 & 1.91 & BLL & HBL & VLT & 55191\\
2FGL J0647.8$-$6102 & 101.920750 & $-$60.967972 & J0647$-$6058 & 0.37$\pm$0.12 & $-$0.991$\pm$0.807 & ... & ... & . & ... & 0.48 & 0.54 & 6.96 & UNK & . & NTT & 55205\\
2FGL J0650.7+2505 & 102.693450 & 25.049886 & J0650+2502 & 2.24$\pm$0.12 & $-$0.789$\pm$0.215 & ... & ... & . & ... & 0.49 & 0.59 & 1.63 & BLL & HBL & WMKO & 55475\\
2FGL J0700.3$-$6611 & 105.130000 & $-$66.179500 & J0700$-$6610 & 2.35$\pm$0.11 & $-$0.845$\pm$0.004 & ... & ... & . & ... & 0.39 & 0.51 & 1.92 & BLL & IBL & VLT & 55191\\
2FGL J0702.7$-$1951 & 105.678826 & $-$19.856461 & J0702$-$1951 & 1.71$\pm$0.12 & $-$0.882$\pm$0.099 & ... & ... & . & ... & 0.42 & 0.46 & 1.68 & BLL & . & WMKO & 55476\\
2FGL J0706.5+3744 & 106.631957 & 37.743489 & J0706+3744 & 1.64$\pm$0.11 & $-$0.792$\pm$0.072 & ... & ... & . & ... & 0.71 & 0.79 & 1.63 & BLL & HBL & WMKO & 55547\\
2FGL J0706.5+7741 & 106.713674 & 77.693491 & J0706+7741 & 2.03$\pm$0.11 & $-$0.946$\pm$0.047 & ... & ... & . & ... & 0.39 & 0.43 & 1.76 & BLL & IBL & P200 & 55567\\
2FGL J0709.3$-$0256 & 107.437581 & $-$2.921523 & J0709$-$0255 & 0.71$\pm$0.12 & $-$2.002$\pm$0.553 & ... & 1.472: & N & 0.785 & 0.64 & 0.73 & 3.09 & BLL & . & WMKO & 55547\\
2FGL J0712.9+5032 & 108.182273 & 50.556308 & J0712+5033 & 1.23$\pm$0.11 & $-$1.470$\pm$0.006 & $-$22.01$\pm$0.22 & 0.502 & G & ... & 0.50 & 0.86 & 1.67 & BLL & LBL & WMKO & 55547\\
2FGL J0718.7$-$4320 & 109.680875 & $-$43.330694 & J0718$-$4319 & 1.99$\pm$0.11 & $-$0.654$\pm$0.024 & ... & ... & . & ... & 0.47 & 0.52 & 1.99 & BLL & IBL & VLT & 55191\\
2FGL J0721.9+7120 & 110.471254 & 71.343499 & J0721+7120 & 2.82$\pm$0.11 & $-$1.581$\pm$0.013 & ... & ... & . & ... & 0.14 & 0.23 & 2.61 & BLL & IBL & HET & 53795\\
2FGL J0753.0+5352 & 118.256064 & 53.883128 & J0753+5352 & 1.26$\pm$0.11 & $-$1.081$\pm$0.116 & ... & ... & . & ... & 0.42 & 0.54 & 1.94 & BLL & LBL & P200 & 55567\\
2FGL J0754.4$-$1147 & 118.610422 & $-$11.787854 & J0754$-$1147 & 1.31$\pm$0.12 & $-$0.401$\pm$0.068 & ... & ... & . & ... & 0.37 & 0.49 & 2.77 & BLL & . & HET & 55267\\
2FGL J0754.8+4824 & 118.690256 & 48.397256 & J0754+4823 & 1.87$\pm$0.11 & $-$1.453$\pm$0.004 & ... & ... & . & 0.889 & 0.34 & 0.53 & 2.17 & BLL & IBL & SDSS & 53089\\
2FGL J0801.5+4401 & 120.284447 & 44.019536 & J0801+4401 & 0.48$\pm$0.2 & $-$1.384$\pm$0.149 & ... & ... & . & ... & 0.51 & 0.54 & 3.23 & BLL & . & HET & 55319\\
2FGL J0807.1$-$0543 & 121.790059 & $-$5.687072 & J0807$-$0541 & 1.34$\pm$0.12 & $-$1.194$\pm$0.010 & ... & ... & . & ... & 0.69 & 0.92 & 1.64 & BLL & . & WMKO & 55547\\
2FGL J0809.8+5218 & 122.455145 & 52.316117 & J0809+5218 & 2.54$\pm$0.11 & $-$0.612$\pm$0.008 & $-$22.6$\pm$0.19 & 0.137 & G & ... & 0.14 & 0.14 & 2.22 & BLL & HBL & SDSS & 53297\\
2FGL J0811.1$-$7527 & 122.763625 & $-$75.507639 & J0811$-$7530 & 1.95$\pm$0.11 & $-$0.779$\pm$0.070 & ... & ... & . & 0.689 & 0.19 & 0.60 & 1.91 & BLL & IBL & VLT & 55191\\
2FGL J0814.7+6429 & 123.663782 & 64.522528 & J0814+6431 & 1.99$\pm$0.11 & $-$1.273$\pm$0.002 & $-$21.32$\pm$0.23 & 0.239 & B & ... & 0.59 & 0.59 & 1.64 & BLL & IBL & WMKO & 55475\\
2FGL J0816.4$-$1311 & 124.112735 & $-$13.197964 & J0816$-$1311 & 1.97$\pm$0.12 & $-$0.294$\pm$0.047 & ... & ... & . & ... & 0.28 & 0.34 & 1.66 & BLL & HBL & WMKO & 55476\\
2FGL J0816.5+5739 & 124.094512 & 57.652517 & J0816+5739 & 1.66$\pm$0.12 & $-$1.021$\pm$0.210 & ... & ... & . & ... & 0.40 & 0.52 & 2.16 & BLL & HBL & SDSS & 54437\\
2FGL J0818.2$-$0935 & 124.457391 & $-$9.558391 & J0817$-$0933 & 1.69$\pm$0.11 & $-$1.605$\pm$0.029 & ... & ... & . & 0.567 & 0.28 & 0.35 & 2.15 & BLL & . & P200 & 54450\\
2FGL J0818.2+4223 & 124.566752 & 42.379383 & J0818+4222 & 1.61$\pm$0.12 & $-$1.411$\pm$0.082 & ... & ... & . & ... & 0.37 & 0.46 & 2.47 & BLL & LBL & HET & 55479\\
2FGL J0819.3+2750 & 124.828715 & 27.791893 & J0819+2747 & 0.92$\pm$0.11 & $-$1.726$\pm$0.019 & ... & ... & . & ... & 0.49 & 0.60 & 2.50 & BLL & . & SDSS & 52670\\
2FGL J0825.9+0308 & 126.459874 & 3.156870 & J0825+0309 & 1.04$\pm$0.18 & $-$1.336$\pm$0.447 & ... & 0.505: & N & ... & 0.42 & 0.42 & 3.21 & BLL & IBL & HET & 55510\\
2FGL J0831.9+0429 & 127.953711 & 4.493993 & J0831+0429 & 2.2$\pm$0.11 & $-$1.168$\pm$0.009 & $-$22.31$\pm$0.20 & 0.174 & G & ... & 0.17 & 0.44 & 2.19 & BLL & LBL & SDSS & 52646\\
2FGL J0834.3+4400 & 128.742630 & 44.060538 & J0834+4403 & 1.15$\pm$0.11 & $-$1.560$\pm$0.198 & ... & ... & . & ... & 0.51 & 0.60 & 2.17 & BLL & . & SDSS & 52232\\
2FGL J0839.4+1802 & 129.878040 & 18.046445 & J0839+1802 & 1.79$\pm$0.12 & $-$1.467$\pm$0.037 & ... & ... & . & ... & 0.42 & 0.42 & 2.17 & BLL & IBL & SDSS & 53711\\
2FGL J0839.7+3541 & 129.930985 & 35.666968 & J0839+3540 & 1.06$\pm$0.11 & $-$1.316$\pm$0.069 & ... & ... & . & ... & 0.50 & 0.50 & 2.19 & BLL & . & SDSS & 52320\\
2FGL J0843.9+5312 & 131.049024 & 53.213882 & J0844+5312 & 1.38$\pm$0.13 & $-$1.262$\pm$0.207 & ... & ... & . & ... & 0.39 & 0.43 & 2.51 & BLL & IBL & HET & 55482\\
2FGL J0848.1$-$0703 & 131.986571 & $-$7.055007 & J0847$-$0703 & 2.12$\pm$0.11 & $-$1.210$\pm$0.019 & ... & ... & . & ... & 0.38 & 0.38 & 2.44 & BLL & IBL & HET & 54780\\
2FGL J0847.0$-$2334 & 131.756549 & $-$23.617120 & J0847$-$2337 & 1.59$\pm$0.12 & $-$0.928$\pm$0.109 & $-$22.28$\pm$0.20 & 0.059 & G & ... & 0.06 & 0.23 & 2.51 & BLL & . & NTT & 55205\\
2FGL J0847.2+1134 & 131.803913 & 11.563984 & J0847+1133 & 1.35$\pm$0.11 & $-$0.629$\pm$0.026 & $-$22.3$\pm$0.13 & 0.198 & G & ... & 0.20 & 0.56 & 2.17 & BLL & HBL & SDSS & 53801\\
2FGL J0849.2+6606 & 132.228082 & 66.102454 & J0848+6606 & 1.43$\pm$0.11 & $-$0.980$\pm$0.012 & ... & ... & . & ... & 0.47 & 0.60 & 2.17 & BLL & . & P200 & 55152\\
2FGL J0849.0+0455 & 132.385242 & 4.918602 & J0849+0455 & 1.38$\pm$0.12 & $-$1.225$\pm$0.215 & ... & ... & . & ... & 0.45 & 0.59 & 1.76 & BLL & . & SDSS & 52670\\
2FGL J0856.6$-$1105 & 134.174372 & $-$11.087273 & J0856$-$1105 & 1.84$\pm$0.12 & $-$1.686$\pm$0.004 & ... & ... & . & 1.397 & 0.31 & 0.38 & 2.18 & BLL & LBL & WMKO & 54790\\
2FGL J0856.3+2058 & 134.165836 & 20.962279 & J0856+2057 & 1.27$\pm$0.11 & $-$1.250$\pm$0.111 & ... & ... & . & ... & 0.46 & 0.54 & 1.64 & BLL & . & SDSS & 53683\\
2FGL J0902.4+2050 & 135.611961 & 20.846000 & J0902+2050 & 2.12$\pm$0.11 & $-$1.208$\pm$0.063 & ... & ... & . & ... & 0.40 & 0.41 & 2.18 & BLL & IBL & SDSS & 53708\\
2FGL J0905.6+1357 & 136.396130 & 13.967697 & J0905+1358 & 2.03$\pm$0.11 & $-$0.860$\pm$0.200 & ... & ... & . & ... & 0.47 & 0.63 & 1.64 & BLL & . & WMKO & 55358\\
2FGL J0906.2$-$0906 & 136.575379 & $-$9.095587 & J0906$-$0905 & 1.82$\pm$0.11 & $-$1.000$\pm$0.041 & ... & ... & . & ... & 0.39 & 0.39 & 2.47 & BLL & . & HET & 55615\\
2FGL J0909.6+0158 & 137.416055 & 2.001422 & J0909+0200 & 1.15$\pm$0.12 & $-$1.300$\pm$0.050 & ... & ... & . & ... & 0.59 & 0.81 & 2.16 & BLL & . & HET & 54892\\
2FGL J0909.2+2308 & 137.252977 & 23.186662 & J0909+2311 & 1.43$\pm$0.11 & $-$1.238$\pm$0.015 & ... & ... & . & 0.431 & 0.48 & 0.55 & 2.52 & BLL & HBL & SDSS & 53708\\
2FGL J0910.6+3329 & 137.655162 & 33.490252 & J0910+3329 & 2.1$\pm$0.11 & $-$0.649$\pm$0.112 & ... & ... & . & ... & 0.28 & 0.39 & 1.77 & BLL & HBL & P200 & 55567\\
2FGL J0912.5+2758 & 138.046700 & 27.991100 & J0912+2759 & 0.95$\pm$0.11 & $-$1.037$\pm$0.012 & ... & ... & . & ... & 0.52 & 0.60 & 2.31 & BLL & HBL & SDSS & 53388\\
2FGL J0915.8+2932 & 138.968343 & 29.556674 & J0915+2933 & 1.53$\pm$0.11 & $-$1.279$\pm$0.025 & ... & ... & . & ... & 0.48 & 0.53 & 1.69 & BLL & HBL & WMKO & 55357\\
2FGL J0921.9+2335 & 140.438990 & 23.596781 & J0921+2335 & 1.45$\pm$0.11 & $-$1.043$\pm$0.194 & ... & ... & . & ... & 0.52 & 0.53 & 2.17 & BLL & . & SDSS & 53714\\
2FGL J0929.5+5009 & 142.314713 & 50.226509 & J0929+5013 & 1.48$\pm$0.12 & $-$0.877$\pm$0.078 & ... & ... & . & ... & 0.39 & 0.54 & 1.77 & BLL & IBL & P200 & 55567\\
2FGL J0930.4+8611 & 142.428528 & 86.205911 & J0929+8612 & 1.5$\pm$0.11 & $-$1.394$\pm$0.028 & ... & ... & . & ... & 0.34 & 0.39 & 2.17 & BLL & LBL & P200 & 55567\\
2FGL J0934.7+3932 & 143.527628 & 39.442425 & J0934+3926 & 1.26$\pm$0.11 & $-$1.385$\pm$0.088 & ... & ... & . & ... & 0.44 & 0.53 & 2.19 & BLL & . & SDSS & 52725\\
2FGL J0941.4+6148 & 145.093673 & 61.806955 & J0940+6148 & 0.98$\pm$0.12 & $-$1.405$\pm$0.045 & $-$22.5$\pm$0.10 & 0.211 & G & ... & 0.21 & 0.21 & 3.35 & BLL & HBL & SDSS & 51910\\
2FGL J0941.4+2724 & 145.468463 & 27.371586 & J0941+2722 & 0.81$\pm$0.13 & $-$2.023$\pm$0.498 & ... & ... & . & ... & 0.37 & 0.43 & 2.19 & BLL & LBL & HET & 55511\\
2FGL J0941.9$-$0755 & 145.589392 & $-$7.998102 & J0942$-$0759 & 1.03$\pm$0.11 & $-$1.847$\pm$0.044 & ... & ... & . & ... & 0.46 & 0.46 & 2.38 & BLL & . & P200 & 54451\\
2FGL J0945.9+5751 & 146.426223 & 57.962795 & J0945+5757 & 1.5$\pm$0.11 & $-$1.134$\pm$0.018 & $-$22.76$\pm$0.09 & 0.229 & G & ... & 0.23 & 0.23 & 2.17 & BLL & . & SDSS & 51915\\
2FGL J0950.1+4554 & 147.549427 & 45.888649 & J0950+4553 & 1.15$\pm$0.12 & $-$1.481$\pm$0.009 & ... & ... & . & ... & 0.40 & 0.58 & 2.17 & BLL & IBL & SDSS & 54525\\
2FGL J0953.1$-$0839 & 148.261238 & $-$8.671821 & J0953$-$0840 & 1.66$\pm$0.11 & $-$0.897$\pm$0.047 & ... & ... & . & ... & 0.59 & 0.59 & 1.64 & BLL & HBL & WMKO & 55547\\
2FGL J1007.7+0621 & 152.003465 & 6.356039 & J1008+0621 & 1.11$\pm$0.11 & $-$1.937$\pm$0.014 & ... & ... & . & ... & 0.54 & 0.58 & 2.17 & BLL & LBL & WMKO & 55357\\
2FGL J1012.1+0631 & 153.055881 & 6.515617 & J1012+0630 & 1.56$\pm$0.12 & $-$1.147$\pm$0.213 & ... & ... & . & 0.516 & 0.49 & 0.49 & 2.16 & BLL & IBL & SDSS & 52641\\
2FGL J1012.5+4227 & 153.184273 & 42.499051 & J1012+4229 & 1.15$\pm$0.11 & $-$0.871$\pm$0.028 & $-$22.82$\pm$0.10 & 0.365 & G & ... & 0.36 & 0.36 & 2.16 & BLL & HBL & SDSS & 54941\\
2FGL J1019.0+5915 & 154.744232 & 59.191048 & J1018+5911 & 1.39$\pm$0.11 & $-$1.302$\pm$0.067 & ... & ... & . & ... & 0.53 & 0.63 & 2.17 & BLL & IBL & SDSS & 52316\\
2FGL J1019.8+6322 & 154.962082 & 63.333971 & J1019+6320 & 1.41$\pm$0.11 & $-$1.185$\pm$0.007 & ... & ... & . & ... & 0.52 & 0.52 & 1.78 & BLL & . & P200 & 55567\\
2FGL J1023.1$-$0115 & 155.682369 & $-$1.217172 & J1022$-$0113 & 1.4$\pm$0.12 & $-$0.369$\pm$0.176 & ... & ... & . & ... & 0.39 & 0.40 & 1.80 & BLL & HBL & P200 & 55567\\
2FGL J1023.8$-$4335 & 155.983417 & $-$43.600000 & J1023$-$4336 & 1.89$\pm$0.11 & $-$0.307$\pm$0.013 & ... & ... & . & ... & 0.34 & 0.39 & 2.24 & BLL & HBL & NTT & 55205\\
2FGL J1026.3$-$8546 & 156.643292 & $-$85.720778 & J1026$-$8543 & 1.59$\pm$0.11 & $-$0.673$\pm$0.201 & ... & ... & . & ... & 0.32 & 0.46 & 2.30 & BLL & LBL & NTT & 55205\\
2FGL J1031.0+5053 & 157.827146 & 50.893557 & J1031+5053 & 1.86$\pm$0.12 & $-$0.666$\pm$0.156 & ... & ... & . & ... & 0.36 & 0.36 & 2.17 & BLL & HBL & SDSS & 52707\\
2FGL J1032.6+3733 & 158.169720 & 37.640764 & J1032+3738 & 1.49$\pm$0.12 & $-$1.060$\pm$0.086 & ... & ... & . & 0.528 & 0.47 & 0.57 & 2.17 & BLL & . & SDSS & 53432\\
2FGL J1037.6+5712 & 159.434512 & 57.198970 & J1037+5711 & 1.44$\pm$0.11 & $-$1.234$\pm$0.007 & ... & ... & . & ... & 0.57 & 0.57 & 1.64 & BLL & IBL & WMKO & 55357\\
2FGL J1049.7+7240 & 161.948623 & 72.636791 & J1047+7238 & 1.63$\pm$0.11 & $-$1.240$\pm$0.150 & ... & ... & . & ... & 0.40 & 0.42 & 2.46 & BLL & . & HET & 55319\\
2FGL J1051.8+0107 & 162.965830 & 1.053453 & J1051+0103 & 0.69$\pm$0.12 & $-$1.126$\pm$0.068 & $-$21.22$\pm$0.18 & 0.265 & G & ... & 0.57 & 0.69 & 2.17 & BLL & IBL & SDSS & 51909\\
2FGL J1051.3+3938 & 162.855863 & 39.723760 & J1051+3943 & 1.13$\pm$0.13 & $-$1.260$\pm$0.317 & ... & ... & . & ... & 0.49 & 0.50 & 2.54 & BLL & HBL & SDSS & 53035\\
2FGL J1053.6+4928 & 163.433429 & 49.498627 & J1053+4929 & 1.43$\pm$0.11 & $-$1.583$\pm$0.030 & $-$22.59$\pm$0.12 & 0.140 & G & ... & 0.14 & 0.14 & 2.17 & BLL & HBL & SDSS & 52669\\
2FGL J1054.5+2212 & 163.627898 & 22.182014 & J1054+2210 & 1.68$\pm$0.11 & $-$1.214$\pm$0.003 & ... & ... & . & ... & 0.51 & 0.63 & 1.64 & BLL & IBL & WMKO & 55358\\
2FGL J1058.6+5628 & 164.657151 & 56.469924 & J1058+5628 & 2.06$\pm$0.11 & $-$0.827$\pm$0.011 & $-$22.32$\pm$0.17 & 0.143 & G & ... & 0.14 & 0.38 & 2.18 & BLL & HBL & SDSS & 52373\\
2FGL J1059.3$-$1132 & 164.801856 & $-$11.572837 & J1059$-$1134 & 1.93$\pm$0.11 & $-$1.473$\pm$0.013 & ... & ... & . & ... & 0.53 & 0.53 & 1.65 & BLL & LBL & WMKO & 55358\\
2FGL J1103.9$-$5356 & 165.967540 & $-$53.950222 & J1103$-$5357 & 2.02$\pm$0.11 & $-$2.223$\pm$0.299 & ... & ... & . & ... & 0.15 & 0.24 & 2.27 & BLL & LBL & SOAR & 56010\\
2FGL J1104.3+0729 & 166.100351 & 7.514478 & J1104+0730 & 1.57$\pm$0.11 & $-$0.747$\pm$0.001 & ... & ... & . & ... & 0.68 & 0.79 & 1.65 & BLL & . & WMKO & 55358\\
2FGL J1107.5+0223 & 166.899968 & 2.373750 & J1107+0222 & 1.07$\pm$0.12 & $-$1.109$\pm$0.122 & ... & ... & . & 1.075 & 0.48 & 0.48 & 2.20 & BLL & . & SDSS & 52374\\
2FGL J1107.8+1505 & 166.950586 & 15.036293 & J1107+1502 & 1.42$\pm$0.12 & $-$0.838$\pm$0.186 & ... & ... & . & 0.601 & 0.52 & 0.52 & 2.16 & BLL & HBL & SDSS & 53377\\
2FGL J1109.3+2414 & 167.317595 & 24.188976 & J1109+2411 & 1.27$\pm$0.12 & $-$0.997$\pm$0.286 & ... & ... & . & ... & 0.48 & 0.48 & 2.17 & BLL & . & SDSS & 53857\\
2FGL J1110.1$-$1835 & 167.615363 & $-$18.597586 & J1110$-$1835 & 1.23$\pm$0.11 & $-$0.700$\pm$0.010 & ... & ... & . & ... & 0.51 & 0.58 & 2.23 & BLL & LBL & NTT & 55205\\
2FGL J1117.2+2013 & 169.276058 & 20.235491 & J1117+2014 & 1.78$\pm$0.11 & $-$1.142$\pm$0.018 & $-$22.14$\pm$0.15 & 0.138 & G & ... & 0.14 & 0.40 & 2.17 & BLL & HBL & SDSS & 54175\\
2FGL J1118.0+5354 & 169.488442 & 53.931499 & J1117+5355 & 1.78$\pm$0.11 & $-$0.791$\pm$0.071 & ... & ... & . & 0.720 & 0.21 & 0.55 & 2.17 & BLL & HBL & SDSS & 52707\\
2FGL J1121.0+4211 & 170.200240 & 42.203931 & J1120+4212 & 1.78$\pm$0.11 & $-$0.577$\pm$0.199 & ... & ... & . & ... & 0.43 & 0.48 & 2.17 & BLL & HBL & SDSS & 53084\\
2FGL J1125.2+4933 & 171.223992 & 49.569776 & J1124+4934 & 1.12$\pm$0.12 & $-$1.022$\pm$0.186 & ... & ... & . & ... & 0.46 & 0.59 & 2.20 & BLL & HBL & SDSS & 52438\\
2FGL J1125.6$-$3559 & 171.380514 & $-$35.951387 & J1125$-$3557 & 1.91$\pm$0.11 & $-$1.097$\pm$0.004 & $-$21.32$\pm$0.37 & 0.284 & B & ... & 0.39 & 0.39 & 1.93 & BLL & IBL & VLT & 55191\\
2FGL J1132.9+0033 & 173.190197 & 0.574423 & J1132+0034 & 1.38$\pm$0.11 & $-$1.180$\pm$0.006 & $-$22.67$\pm$0.31 & 0.678 & N & ... & 0.60 & 0.68 & 1.86 & BLL & IBL & WMKO & 55358\\
2FGL J1136.3+6736 & 174.124687 & 67.618288 & J1136+6737 & 1.43$\pm$0.11 & $-$1.264$\pm$0.026 & $-$22.52$\pm$0.13 & 0.134 & G & ... & 0.13 & 0.13 & 2.16 & BLL & HBL & SDSS & 51955\\
2FGL J1141.9+1550 & 175.532295 & 15.798248 & J1142+1547 & 0.89$\pm$0.13 & $-$1.238$\pm$0.127 & ... & ... & . & ... & 0.45 & 0.46 & 3.11 & BLL & . & HET & 55615\\
2FGL J1143.1+6119 & 175.800416 & 61.369731 & J1143+6122 & 1.41$\pm$0.11 & $-$1.253$\pm$0.017 & ... & ... & . & ... & 0.41 & 0.53 & 2.18 & BLL & . & SDSS & 52319\\
2FGL J1150.1+2419 & 177.580100 & 24.298214 & J1150+2417 & 1.06$\pm$0.11 & $-$1.080$\pm$0.100 & ... & ... & . & ... & 0.32 & 0.39 & 2.21 & BLL & LBL & P200 & 55567\\
2FGL J1150.5+4154 & 177.644398 & 41.911636 & J1150+4154 & 1.4$\pm$0.12 & $-$1.254$\pm$0.145 & ... & ... & . & ... & 0.54 & 0.70 & 1.66 & BLL & HBL & WMKO & 55357\\
2FGL J1151.5$-$1347 & 177.875089 & $-$13.797539 & J1151$-$1347 & 1.03$\pm$0.11 & $-$1.211$\pm$0.005 & ... & ... & . & 0.838 & 0.30 & 0.84 & 2.16 & BLL & . & WMKO & 55358\\
2FGL J1151.5+5857 & 177.852769 & 58.988465 & J1151+5859 & 1.82$\pm$0.11 & $-$0.871$\pm$0.001 & ... & ... & . & ... & 0.54 & 0.59 & 1.76 & BLL & IBL & P200 & 55152\\
2FGL J1154.0$-$0010 & 178.517941 & $-$0.169121 & J1154$-$0010 & 0.93$\pm$0.12 & $-$0.889$\pm$0.051 & $-$22.35$\pm$0.10 & 0.254 & G & ... & 0.25 & 0.25 & 2.22 & BLL & HBL & SDSS & 51943\\
2FGL J1203.2+6030 & 180.764820 & 60.522024 & J1203+6031 & 2.2$\pm$0.11 & $-$1.214$\pm$0.014 & $-$22.03$\pm$0.10 & 0.065 & G & ... & 0.07 & 0.26 & 2.18 & BLL & IBL & SDSS & 52405\\
2FGL J1204.2+1144 & 181.050729 & 11.765358 & J1204+1145 & 1.46$\pm$0.11 & $-$0.824$\pm$0.018 & $-$22.59$\pm$0.08 & 0.296 & G & ... & 0.30 & 0.30 & 2.17 & BLL & HBL & SDSS & 53147\\
2FGL J1209.6+4121 & 182.345107 & 41.328043 & J1209+4119 & 1.57$\pm$0.11 & $-$0.875$\pm$0.115 & ... & ... & . & ... & 0.35 & 0.54 & 1.78 & BLL & LBL & P200 & 55567\\
2FGL J1214.9+5004 & 183.753508 & 50.037813 & J1215+5002 & 1.13$\pm$0.11 & $-$0.960$\pm$0.264 & ... & ... & . & ... & 0.54 & 0.67 & 1.82 & BLL & . & P200 & 55335\\
2FGL J1218.5$-$0122 & 184.645454 & $-$1.331449 & J1218$-$0119 & 2.2$\pm$0.11 & $-$1.018$\pm$0.003 & ... & ... & . & 0.642 & 0.30 & 0.32 & 1.64 & BLL & . & WMKO & 55358\\
2FGL J1219.8$-$0310 & 184.940437 & $-$3.239303 & J1219$-$0314 & 1.43$\pm$0.11 & $-$1.086$\pm$0.022 & $-$22.6$\pm$0.10 & 0.299 & G & ... & 0.30 & 0.30 & 2.19 & BLL & HBL & SDSS & 52313\\
2FGL J1221.4+2814 & 185.381706 & 28.232836 & J1221+2813 & 2.63$\pm$0.11 & $-$1.118$\pm$0.006 & $-$21.35$\pm$0.25 & 0.103 & N & ... & 0.26 & 0.28 & 2.22 & BLL & IBL & SDSS & 53816\\
2FGL J1221.3+3010 & 185.341328 & 30.176754 & J1221+3010 & 2.06$\pm$0.11 & $-$0.772$\pm$0.009 & $-$22.42$\pm$0.17 & 0.184 & G & ... & 0.18 & 0.18 & 2.18 & BLL & HBL & SDSS & 53799\\
2FGL J1223.9+8043 & 185.918955 & 80.667944 & J1223+8040 & 0.57$\pm$0.12 & $-$1.513$\pm$0.150 & ... & ... & . & ... & 0.43 & 0.51 & 3.74 & BLL & LBL & P200 & 55064\\
2FGL J1225.0+4335 & 186.214684 & 43.589085 & J1224+4335 & 0.83$\pm$0.12 & $-$1.714$\pm$0.261 & ... & ... & . & 0.703 & 0.52 & 0.61 & 2.27 & BLL & . & SDSS & 53112\\
2FGL J1226.7$-$1331 & 186.726778 & $-$13.477455 & J1226$-$1328 & 1.43$\pm$0.11 & $-$1.832$\pm$0.018 & ... & ... & . & ... & 0.40 & 0.40 & 1.76 & BLL & . & WMKO & 54470\\
2FGL J1230.2+2517 & 187.558728 & 25.302083 & J1230+2518 & 1.92$\pm$0.11 & $-$1.158$\pm$0.015 & ... & ... & . & ... & 0.32 & 0.39 & 1.78 & BLL & IBL & P200 & 55567\\
2FGL J1231.7+2848 & 187.932711 & 28.797518 & J1231+2847 & 2.13$\pm$0.12 & $-$0.983$\pm$0.002 & ... & 0.236: & N & ... & 0.30 & 0.47 & 2.18 & BLL & HBL & SDSS & 53823\\
2FGL J1233.7$-$0145 & 188.422913 & $-$1.740585 & J1233$-$0144 & 1.08$\pm$0.12 & $-$0.988$\pm$0.137 & ... & ... & . & ... & 0.43 & 0.51 & 2.50 & BLL & . & HET & 55323\\
2FGL J1243.1+3627 & 190.802908 & 36.462495 & J1243+3627 & 2.21$\pm$0.11 & $-$0.891$\pm$0.084 & ... & ... & . & 0.485 & 0.34 & 0.38 & 1.77 & BLL & HBL & P200 & 55336\\
2FGL J1245.1+5708 & 191.291570 & 57.165173 & J1245+5709 & 1.76$\pm$0.11 & $-$1.269$\pm$0.048 & ... & ... & . & 0.522 & 0.48 & 0.52 & 2.17 & BLL & IBL & SDSS & 52765\\
2FGL J1248.2+5820 & 192.078231 & 58.341312 & J1248+5820 & 2.04$\pm$0.11 & $-$0.903$\pm$0.012 & ... & ... & . & ... & 0.41 & 0.46 & 1.64 & BLL & IBL & WMKO & 55357\\
2FGL J1249.9+3705 & 192.444585 & 37.130830 & J1249+3707 & 1.11$\pm$0.11 & $-$0.674$\pm$0.094 & ... & ... & . & ... & 0.55 & 0.61 & 2.19 & BLL & HBL & SDSS & 53772\\
2FGL J1251.2+1045 & 192.824537 & 10.651445 & J1251+1039 & 1.34$\pm$0.12 & $-$0.972$\pm$0.033 & $-$22.05$\pm$0.16 & 0.245 & G & ... & 0.25 & 0.49 & 2.17 & BLL & HBL & SDSS & 54266\\
2FGL J1253.1+5302 & 193.299770 & 53.019997 & J1253+5301 & 1.68$\pm$0.12 & $-$1.354$\pm$0.102 & ... & ... & . & 0.663 & 0.55 & 0.55 & 1.64 & BLL & IBL & WMKO & 55357\\
2FGL J1254.1+6237 & 193.497605 & 62.715855 & J1253+6242 & 1.29$\pm$0.12 & $-$1.501$\pm$0.300 & ... & ... & . & 0.867 & 0.48 & 0.58 & 2.18 & BLL & HBL & SDSS & 52320\\
2FGL J1254.4+2209 & 193.638712 & 22.184153 & J1254+2211 & 1.74$\pm$0.12 & $-$0.978$\pm$0.156 & ... & ... & . & ... & 0.42 & 0.51 & 2.17 & BLL & . & SDSS & 54212\\
2FGL J1257.0+3650 & 194.318917 & 36.787496 & J1257+3647 & 1.38$\pm$0.11 & $-$0.896$\pm$0.018 & $-$23.14$\pm$0.25 & 0.531 & G & ... & 0.51 & 0.53 & 2.16 & BLL & HBL & SDSS & 53848\\
2FGL J1303.1+2435 & 195.763523 & 24.565348 & J1303+2433 & 2.05$\pm$0.11 & $-$1.389$\pm$0.048 & ... & ... & . & 0.769 & 0.25 & 0.28 & 1.69 & BLL & . & WMKO & 55039\\
2FGL J1304.3$-$4353 & 196.087167 & $-$43.885639 & J1304$-$4353 & 2.24$\pm$0.12 & $-$0.083$\pm$0.098 & ... & ... & . & ... & 0.17 & 0.17 & 2.12 & BLL & HBL & SOAR & 56010\\
2FGL J1309.3+1154 & 197.391406 & 11.906687 & J1309+1154 & 1.28$\pm$0.12 & $-$1.561$\pm$0.015 & ... & ... & . & ... & 0.56 & 0.56 & 2.19 & BLL & . & SDSS & 53116\\
2FGL J1309.4+4304 & 197.356580 & 43.084824 & J1309+4305 & 1.67$\pm$0.12 & $-$1.065$\pm$0.054 & ... & 0.691 & N & ... & 0.46 & 0.58 & 1.80 & BLL & HBL & WMKO & 55357\\
2FGL J1310.9+0036 & 197.776740 & 0.586031 & J1311+0035 & 1.12$\pm$0.12 & $-$0.300$\pm$0.081 & ... & ... & . & ... & 0.33 & 0.37 & 2.79 & BLL & HBL & P200 & 55772\\
2FGL J1312.4$-$2157 & 198.131522 & $-$21.939796 & J1312$-$2156 & 1.73$\pm$0.12 & $-$1.636$\pm$0.103 & ... & 1.600: & B & 1.485 & 0.38 & 0.41 & 1.81 & BLL & . & P200 & 55336\\
2FGL J1314.6+2348 & 198.682487 & 23.807465 & J1314+2348 & 1.96$\pm$0.12 & $-$1.136$\pm$0.019 & ... & ... & . & ... & 0.43 & 0.50 & 4.68 & BLL & IBL & SDSS & 54234\\
2FGL J1314.5$-$5330 & 198.767465 & $-$53.576557 & J1315$-$5334 & 1.13$\pm$0.12 & $-$2.190$\pm$0.881 & ... & ... & . & ... & 0.19 & 0.23 & 2.15 & UNK & . & NTT & 55063\\
2FGL J1326.7$-$5254 & 201.705034 & $-$52.939859 & J1326$-$5256 & 2.25$\pm$0.11 & $-$1.387$\pm$0.004 & ... & ... & . & ... & 0.24 & 0.26 & 2.25 & BLL & LBL & NTT & 55063\\
2FGL J1329.2$-$5608 & 202.254788 & $-$56.133917 & J1329$-$5608 & 1.32$\pm$0.11 & $-$0.839$\pm$0.075 & ... & ... & . & ... & 0.13 & 0.19 & 7.06 & UNK & LBL & NTT & 55065\\
2FGL J1330.9+7001 & 202.607151 & 70.028030 & J1330+7001 & 1.5$\pm$0.14 & $-$0.218$\pm$0.582 & ... & ... & . & ... & 0.43 & 0.51 & 2.10 & BLL & HBL & P200 & 55424\\
2FGL J1338.9+1152 & 204.745948 & 11.888106 & J1338+1153 & 1.24$\pm$0.11 & $-$1.236$\pm$0.084 & ... & ... & . & 1.587 & 0.60 & 0.62 & 1.94 & BLL & . & WMKO & 55357\\
2FGL J1340.5+4407 & 205.122775 & 44.168551 & J1340+4410 & 0.97$\pm$0.12 & $-$1.299$\pm$0.067 & $-$23.56$\pm$0.17 & 0.546 & G & ... & 0.48 & 0.54 & 2.29 & BLL & HBL & SDSS & 52792\\
2FGL J1351.4+1115 & 207.837139 & 11.247959 & J1351+1114 & 1.75$\pm$0.12 & $-$1.197$\pm$0.320 & ... & ... & . & 0.620 & 0.39 & 0.39 & 1.64 & BLL & HBL & WMKO & 55061\\
2FGL J1353.3+1435 & 208.345005 & 14.594318 & J1353+1435 & 1.54$\pm$0.12 & $-$1.742$\pm$0.245 & ... & ... & . & ... & 0.50 & 0.65 & 1.72 & BLL & LBL & WMKO & 55061\\
2FGL J1354.5+3703 & 208.611365 & 37.115096 & J1354+3706 & 1.68$\pm$0.12 & $-$1.072$\pm$0.027 & ... & ... & . & ... & 0.38 & 0.38 & 2.17 & BLL & . & SDSS & 53476\\
2FGL J1358.0+0137 & 209.411224 & 1.470407 & J1357+0128 & 1.63$\pm$0.11 & $-$1.039$\pm$0.004 & ... & ... & . & ... & 0.52 & 0.56 & 2.17 & BLL & HBL & SDSS & 52028\\
2FGL J1359.9$-$3746 & 209.956417 & $-$37.766583 & J1359$-$3746 & 1.88$\pm$0.11 & $-$0.983$\pm$0.009 & $-$22.73$\pm$0.09 & 0.334 & G & ... & 0.33 & 0.33 & 1.91 & BLL & . & VLT & 55191\\
2FGL J1410.3+2811 & 212.622627 & 28.348720 & J1410+2820 & 1.36$\pm$0.12 & $-$1.239$\pm$0.021 & ... & ... & . & ... & 0.49 & 0.49 & 2.17 & BLL & HBL & SDSS & 53793\\
2FGL J1418.1+2539 & 214.484480 & 25.723049 & J1417+2543 & 1.55$\pm$0.11 & $-$0.840$\pm$0.017 & $-$22.94$\pm$0.11 & 0.236 & G & ... & 0.23 & 0.24 & 2.16 & BLL & HBL & SDSS & 53800\\
2FGL J1418.4$-$0234 & 214.610162 & $-$2.560144 & J1418$-$0233 & 2.45$\pm$0.11 & $-$1.052$\pm$0.001 & ... & ... & . & ... & 0.24 & 0.30 & 1.64 & BLL & . & WMKO & 55358\\
2FGL J1420.2+5422 & 214.943774 & 54.387502 & J1419+5423 & 2.37$\pm$0.11 & $-$1.309$\pm$0.007 & $-$22.26$\pm$0.21 & 0.153 & G & ... & 0.15 & 0.36 & 2.19 & BLL & LBL & SDSS & 52762\\
2FGL J1425.1+3615 & 216.231194 & 36.260089 & J1424+3615 & 1.43$\pm$0.11 & $-$1.029$\pm$0.030 & ... & ... & . & ... & 0.46 & 0.57 & 2.17 & BLL & IBL & SDSS & 53144\\
2FGL J1426.1+3406 & 216.531723 & 34.073996 & J1426+3404 & 1.4$\pm$0.11 & $-$1.237$\pm$0.074 & ... & ... & . & ... & 0.77 & 0.84 & 1.63 & BLL & IBL & WMKO & 55040\\
2FGL J1427.4$-$3306 & 216.922612 & $-$33.091976 & J1427$-$3305 & 1.14$\pm$0.11 & $-$1.636$\pm$0.014 & ... & ... & . & ... & 0.48 & 0.51 & 2.40 & BLL & LBL & NTT & 54125\\
2FGL J1427.0+2347 & 216.751606 & 23.800173 & J1427+2347 & 2.79$\pm$0.11 & $-$0.817$\pm$0.006 & ... & ... & . & ... & 0.30 & 0.30 & 1.66 & BLL & HBL & WMKO & 55357\\
2FGL J1428.6+4240 & 217.135609 & 42.672843 & J1428+4240 & 1.64$\pm$0.11 & $-$0.760$\pm$0.024 & $-$22.61$\pm$0.13 & 0.129 & G & ... & 0.13 & 0.13 & 2.18 & BLL & HBL & SDSS & 52825\\
2FGL J1435.1+2022 & 218.841245 & 20.355221 & J1435+2021 & 1.58$\pm$0.11 & $-$1.089$\pm$0.035 & ... & 0.748 & B & ... & 0.41 & 0.41 & 1.63 & BLL & . & WMKO & 55040\\
2FGL J1437.1+5640 & 219.240738 & 56.657022 & J1436+5639 & 1.11$\pm$0.11 & $-$0.683$\pm$0.277 & ... & ... & . & ... & 0.68 & 0.75 & 2.08 & BLL & HBL & WMKO & 55357\\
2FGL J1440.3$-$1540 & 219.987092 & $-$15.530593 & J1439$-$1531 & 1.35$\pm$0.12 & $-$1.546$\pm$0.132 & ... & ... & . & ... & 0.43 & 0.60 & 1.79 & BLL & . & WMKO & 54648\\
2FGL J1440.3+4948 & 219.945593 & 49.968149 & J1439+4958 & 1.53$\pm$0.11 & $-$1.750$\pm$0.138 & ... & ... & . & ... & 0.40 & 0.53 & 2.17 & BLL & IBL & SDSS & 52733\\
2FGL J1440.9+0611 & 220.220920 & 6.170948 & J1440+0610 & 2.29$\pm$0.11 & $-$1.214$\pm$0.012 & ... & ... & . & 0.316 & 0.31 & 0.31 & 1.63 & BLL & IBL & WMKO & 55060\\
2FGL J1442.7+1159 & 220.701101 & 12.011197 & J1442+1200 & 1.54$\pm$0.11 & $-$0.929$\pm$0.021 & $-$22.41$\pm$0.14 & 0.163 & G & ... & 0.16 & 0.16 & 2.17 & BLL & HBL & SDSS & 53531\\
2FGL J1442.0+4352 & 220.531940 & 43.805737 & J1442+4348 & 1.49$\pm$0.11 & $-$1.104$\pm$0.066 & ... & ... & . & 0.674 & 0.44 & 0.56 & 2.17 & BLL & . & SDSS & 52734\\
2FGL J1443.9$-$3908 & 220.987904 & $-$39.143572 & J1443$-$3908 & 2.36$\pm$0.11 & $-$0.960$\pm$0.002 & ... & ... & . & ... & 0.14 & 0.14 & 2.20 & BLL & HBL & NTT & 55063\\
2FGL J1448.0+3608 & 222.002607 & 36.141967 & J1448+3608 & 1.8$\pm$0.12 & $-$0.764$\pm$0.029 & ... & ... & . & 0.738 & 0.46 & 0.60 & 1.76 & BLL & HBL & P200 & 55336\\
2FGL J1451.0+5159 & 222.750118 & 52.019804 & J1451+5201 & 1.07$\pm$0.12 & $-$1.387$\pm$0.012 & ... & 2.471 & S & ... & 0.47 & 0.48 & 2.59 & BLL & . & SDSS & 52786\\
2FGL J1454.4+5123 & 223.613814 & 51.409642 & J1454+5124 & 1.85$\pm$0.11 & $-$1.098$\pm$0.029 & ... & ... & . & ... & 0.46 & 0.63 & 1.63 & BLL & IBL & WMKO & 55357\\
2FGL J1501.0+2238 & 225.257886 & 22.634900 & J1501+2238 & 2.06$\pm$0.11 & $-$1.028$\pm$0.008 & $-$22.2$\pm$0.26 & 0.235 & G & ... & 0.23 & 0.52 & 2.18 & BLL & HBL & SDSS & 54510\\
2FGL J1503.7$-$1541 & 225.919492 & $-$15.688317 & J1503$-$1541 & 1.67$\pm$0.11 & $-$0.589$\pm$0.068 & ... & ... & . & 0.210 & 0.42 & 0.46 & 1.76 & BLL & . & P200 & 55336\\
2FGL J1504.9$-$3433 & 226.259846 & $-$34.549254 & J1505$-$3432 & 0.37$\pm$0.14 & $-$2.032$\pm$0.584 & ... & ... & . & 1.554 & 0.54 & 0.61 & 3.13 & BLL & . & WMKO & 55358\\
2FGL J1508.5+2709 & 227.177881 & 27.152345 & J1508+2709 & 1.2$\pm$0.12 & $-$0.857$\pm$0.034 & $-$22.83$\pm$0.08 & 0.270 & G & ... & 0.27 & 0.27 & 2.19 & BLL & HBL & SDSS & 54523\\
2FGL J1509.7+5556 & 227.449890 & 55.938031 & J1509+5556 & 1.45$\pm$0.12 & $-$1.091$\pm$0.010 & ... & ... & . & ... & 0.50 & 0.58 & 1.76 & BLL & HBL & P200 & 55336\\
2FGL J1516.9+1925 & 229.236701 & 19.537037 & J1516+1932 & 1.29$\pm$0.11 & $-$1.616$\pm$0.005 & ... & ... & . & ... & 0.58 & 0.58 & 1.84 & BLL & . & P200 & 55424\\
2FGL J1518.0+6526 & 229.448127 & 65.423178 & J1517+6525 & 1.47$\pm$0.11 & $-$0.419$\pm$0.079 & ... & ... & . & 0.702 & 0.39 & 0.43 & 1.78 & BLL & HBL & P200 & 55567\\
2FGL J1520.8$-$0349 & 230.203341 & $-$3.813944 & J1520$-$0348 & 1.6$\pm$0.12 & $-$1.039$\pm$0.085 & ... & ... & . & 0.867 & 0.33 & 0.46 & 1.80 & BLL & HBL & P200 & 55424\\
2FGL J1531.0+5725 & 232.743084 & 57.606962 & J1530+5736 & 0.8$\pm$0.12 & $-$0.980$\pm$0.099 & ... & ... & . & ... & 0.62 & 0.64 & 2.31 & BLL & . & SDSS & 52347\\
2FGL J1535.4+3720 & 233.697157 & 37.264974 & J1534+3715 & 1.45$\pm$0.11 & $-$1.100$\pm$0.026 & $-$21.87$\pm$0.16 & 0.144 & G & ... & 0.37 & 0.43 & 2.17 & BLL & IBL & SDSS & 52753\\
2FGL J1540.4+1438 & 235.206293 & 14.796277 & J1540+1447 & 1.52$\pm$0.11 & $-$1.313$\pm$0.015 & $-$22.92$\pm$0.33 & 0.606 & B & ... & 0.50 & 0.50 & 2.16 & BLL & LBL & SDSS & 54567\\
2FGL J1542.9+6129 & 235.737273 & 61.498708 & J1542+6129 & 2.31$\pm$0.11 & $-$1.294$\pm$0.010 & ... & ... & . & ... & 0.34 & 0.34 & 1.76 & BLL & IBL & P200 & 55424\\
2FGL J1546.1+0820 & 236.517907 & 8.320820 & J1546+0819 & 1.64$\pm$0.12 & $-$0.575$\pm$0.202 & ... & ... & . & 0.513 & 0.46 & 0.51 & 2.17 & BLL & HBL & SDSS & 53859\\
2FGL J1548.8$-$2251 & 237.207493 & $-$22.850572 & J1548$-$2251 & 1.94$\pm$0.11 & $-$0.646$\pm$0.007 & $-$22.53$\pm$0.18 & 0.192 & G & ... & 0.19 & 0.19 & 1.65 & BLL & HBL & WMKO & 55358\\
2FGL J1551.9+0855 & 238.013550 & 8.846533 & J1552+0850 & 2.19$\pm$0.11 & $-$1.903$\pm$0.014 & ... & ... & . & 1.209 & 0.21 & 0.29 & 1.66 & BLL & . & WMKO & 55060\\
2FGL J1553.5$-$3116 & 238.389896 & $-$31.308808 & J1553$-$3118 & 2.11$\pm$0.12 & $-$0.408$\pm$0.098 & ... & ... & . & ... & 0.30 & 0.43 & 1.97 & BLL & HBL & VLT & 55055\\
2FGL J1555.7+1111 & 238.929561 & 11.190110 & J1555+1111 & 2.05$\pm$0.11 & $-$0.562$\pm$0.023 & ... & ... & . & ... & 0.24 & 0.31 & 1.77 & BLL & HBL & P200 & 54877\\
2FGL J1559.0+5627 & 239.701256 & 56.420645 & J1558+5625 & 1.79$\pm$0.11 & $-$1.125$\pm$0.014 & ... & ... & . & 0.909 & 0.34 & 0.35 & 2.47 & BLL & IBL & HET & 55590\\
2FGL J1603.8$-$4904 & 240.961170 & $-$49.068221 & J1603$-$4904 & 2.93$\pm$0.12 & $-$0.482$\pm$0.172 & ... & ... & . & ... & ... & ... & 4.24 & BLL & LBL & NTT & 55065\\
2FGL J1604.5$-$4442 & 241.129753 & $-$44.692138 & J1604$-$4441 & 2.19$\pm$0.12 & 0.780$\pm$0.126 & ... & ... & . & ... & 0.01 & 0.03 & 3.94 & UNK & LBL & NTT & 55777\\
2FGL J1610.8$-$6650 & 242.693250 & $-$66.816917 & J1610$-$6649 & 2.42$\pm$0.11 & $-$0.098$\pm$0.036 & ... & ... & . & 0.447 & 0.18 & 0.34 & 1.99 & BLL & HBL & VLT & 55055\\
2FGL J1630.4+5218 & 247.679856 & 52.360729 & J1630+5221 & 1.59$\pm$0.11 & $-$0.716$\pm$0.013 & ... & ... & . & ... & 0.43 & 0.58 & 1.77 & BLL & IBL & P200 & 55064\\
2FGL J1641.6$-$0614 & 250.509183 & $-$6.356516 & J1642$-$0621 & 1.64$\pm$0.11 & $-$1.799$\pm$0.010 & ... & ... & . & ... & 0.20 & 0.35 & 3.14 & BLL & . & HET & 52756\\
2FGL J1643.5$-$0641 & 250.870621 & $-$6.772227 & J1643$-$0646 & 1.62$\pm$0.12 & $-$1.202$\pm$0.056 & $-$21.85$\pm$0.16 & 0.082 & G & ... & 0.28 & 0.30 & 2.07 & BLL & HBL & P200 & 55336\\
2FGL J1649.6+5238 & 252.353892 & 52.587244 & J1649+5235 & 1.88$\pm$0.11 & $-$1.509$\pm$0.007 & ... & ... & . & ... & 0.30 & 0.30 & 2.47 & BLL & . & HET & 55468\\
2FGL J1650.1$-$5044 & 252.569293 & $-$50.746610 & J1650$-$5044 & 1.76$\pm$0.14 & $-$1.328$\pm$0.458 & ... & ... & . & ... & 0.09 & 0.19 & 3.13 & UNK & . & NTT & 55063\\
2FGL J1719.3+1744 & 259.804371 & 17.751828 & J1719+1745 & 1.98$\pm$0.11 & $-$1.397$\pm$0.004 & ... & ... & . & ... & 0.41 & 0.41 & 1.64 & BLL & LBL & WMKO & 55357\\
2FGL J1725.0+1151 & 261.268036 & 11.870948 & J1725+1152 & 2.41$\pm$0.11 & $-$0.803$\pm$0.008 & ... & ... & . & ... & 0.34 & 0.34 & 1.65 & BLL & HBL & WMKO & 55357\\
2FGL J1725.2+5853 & 261.396124 & 58.860884 & J1725+5851 & 1.68$\pm$0.11 & $-$1.243$\pm$0.112 & ... & ... & . & ... & 0.49 & 0.71 & 1.66 & BLL & IBL & WMKO & 55357\\
2FGL J1727.9+1220 & 262.029290 & 12.260864 & J1728+1215 & 0.37$\pm$0.15 & $-$1.488$\pm$0.440 & ... & 0.586 & B & ... & 0.37 & 0.50 & 7.44 & FSRQ & . & HET & 52842\\
2FGL J1731.3+3718 & 262.695334 & 37.248572 & J1730+3714 & 1.3$\pm$0.11 & $-$1.794$\pm$0.029 & $-$22.27$\pm$0.12 & 0.204 & G & ... & 0.20 & 0.53 & 1.80 & BLL & IBL & P200 & 55336\\
2FGL J1731.8$-$3004 & 262.945377 & $-$30.052547 & J1731$-$3003 & 4.25$\pm$0.22 & 1.757$\pm$1.411 & ... & ... & . & ... & ... & ... & 8.23 & BLL & . & NTT & 55778\\
2FGL J1742.1+5948 & 265.633163 & 59.751987 & J1742+5945 & 1.6$\pm$0.11 & $-$1.567$\pm$0.002 & ... & ... & . & ... & 0.48 & 0.48 & 1.76 & BLL & IBL & P200 & 55423\\
2FGL J1745.5$-$0751 & 266.362905 & $-$7.884472 & J1745$-$0753 & 1.55$\pm$0.12 & $-$0.793$\pm$0.072 & ... & ... & . & ... & 0.11 & 0.14 & 3.67 & BLL & LBL & HET & 55311\\
2FGL J1749.1+4323 & 267.250820 & 43.364359 & J1749+4321 & 1.35$\pm$0.11 & $-$1.573$\pm$0.105 & ... & ... & . & 0.571 & 0.75 & 0.78 & 1.65 & BLL & LBL & WMKO & 55475\\
2FGL J1755.5$-$6423 & 268.674667 & $-$64.395750 & J1754$-$6423 & 1.5$\pm$0.11 & $-$1.439$\pm$0.032 & ... & 1.255: & B & ... & 0.38 & 0.43 & 2.26 & BLL & . & NTT & 55776\\
2FGL J1754.3+3212 & 268.549137 & 32.206495 & J1754+3212 & 2.14$\pm$0.11 & $-$1.013$\pm$0.123 & ... & ... & . & ... & 0.58 & 0.58 & 1.63 & BLL & HBL & WMKO & 55475\\
2FGL J1756.5+5523 & 269.066531 & 55.371588 & J1756+5522 & 1.38$\pm$0.11 & $-$0.779$\pm$0.025 & ... & ... & . & 0.657 & 0.65 & 0.68 & 1.65 & BLL & HBL & WMKO & 55357\\
2FGL J1809.4+2042 & 272.356172 & 20.691912 & J1809+2041 & 1.82$\pm$0.11 & $-$0.496$\pm$0.010 & ... & ... & . & 0.280 & 0.33 & 0.34 & 1.83 & BLL & HBL & P200 & 55743\\
2FGL J1809.7+2909 & 272.439086 & 29.172161 & J1809+2910 & 1.71$\pm$0.11 & $-$1.127$\pm$0.012 & ... & ... & . & ... & 0.60 & 0.69 & 1.63 & BLL & . & WMKO & 55040\\
2FGL J1810.8+1606 & 272.709048 & 16.138925 & J1810+1608 & 1.2$\pm$0.11 & $-$0.999$\pm$0.095 & ... & ... & . & ... & 0.75 & 0.90 & 1.74 & BLL & . & WMKO & 55040\\
2FGL J1813.7+0617 & 273.389089 & 6.261734 & J1813+0615 & 1.96$\pm$0.12 & $-$1.503$\pm$0.050 & ... & ... & . & 1.038 & 0.17 & 0.23 & 2.64 & BLL & . & HET & 53862\\
2FGL J1823.7+6856 & 275.887119 & 68.964465 & J1823+6857 & 1.36$\pm$0.12 & $-$1.488$\pm$0.031 & ... & ... & . & ... & 0.21 & 0.38 & 3.35 & BLL & LBL & HET & 53219\\
2FGL J1824.0+5650 & 276.029528 & 56.850312 & J1824+5651 & 1.91$\pm$0.11 & $-$1.696$\pm$0.021 & ... & 0.664 & B & ... & 0.30 & 0.39 & 2.48 & BLL & LBL & HET & 55329\\
2FGL J1829.3$-$2419 & 277.228422 & $-$24.293682 & J1828$-$2417 & 1.62$\pm$0.12 & $-$0.993$\pm$0.223 & ... & ... & . & ... & 0.04 & 0.04 & 1.75 & UNK & HBL & NTT & 55776\\
2FGL J1829.1+2725 & 277.308371 & 27.484193 & J1829+2729 & 2.18$\pm$0.13 & $-$0.555$\pm$0.734 & ... & ... & . & ... & 0.20 & 0.27 & 4.43 & UNK & . & HET & 55706\\
2FGL J1829.2+5402 & 277.351707 & 54.049936 & J1829+5402 & 1.55$\pm$0.11 & $-$0.916$\pm$0.010 & ... & ... & . & ... & 0.57 & 0.57 & 2.46 & BLL & HBL & P200 & 55423\\
2FGL J1830.0+1325 & 277.503139 & 13.403874 & J1830+1324 & 1.43$\pm$0.11 & $-$1.027$\pm$0.052 & ... & ... & . & ... & 0.66 & 0.71 & 1.66 & BLL & . & WMKO & 55476\\
2FGL J1832.7$-$5700 & 278.128750 & $-$56.989222 & J1832$-$5659 & 1.43$\pm$0.11 & $-$0.776$\pm$0.055 & ... & ... & . & 1.227 & 0.42 & 0.57 & 1.96 & BLL & . & VLT & 55056\\
2FGL J1836.2+3137 & 279.088399 & 31.607098 & J1836+3136 & 1.57$\pm$0.11 & $-$1.363$\pm$0.008 & ... & ... & . & ... & 0.32 & 0.54 & 1.76 & BLL & HBL & P200 & 55423\\
2FGL J1844.7+5716 & 281.213316 & 57.161254 & J1844+5709 & 1.68$\pm$0.11 & $-$1.363$\pm$0.024 & ... & ... & . & ... & 0.35 & 0.44 & 2.48 & BLL & . & HET & 55735\\
2FGL J1849.7$-$4310 & 282.357083 & $-$43.237278 & J1849$-$4314 & 2.03$\pm$0.11 & $-$0.782$\pm$0.031 & ... & ... & . & ... & 0.38 & 0.46 & 1.94 & BLL & . & VLT & 55056\\
2FGL J1849.5+2744 & 282.382041 & 27.800246 & J1849+2748 & 1.47$\pm$0.12 & $-$1.892$\pm$0.057 & ... & ... & . & 1.466 & 0.29 & 0.31 & 2.50 & BLL & . & HET & 55478\\
2FGL J1903.3+5539 & 285.798229 & 55.677497 & J1903+5540 & 2.1$\pm$0.11 & $-$1.161$\pm$0.004 & ... & ... & . & 0.727 & 0.43 & 0.58 & 1.63 & BLL & IBL & WMKO & 55475\\
2FGL J1912.0+1609 & 287.992584 & 16.196460 & J1911+1611 & 1.54$\pm$0.16 & 0.689$\pm$0.416 & ... & ... & . & ... & 0.01 & 0.03 & 5.51 & UNK & . & HET & 55752\\
2FGL J1918.2$-$4110 & 289.566708 & $-$41.191944 & J1918$-$4111 & 1.62$\pm$0.11 & $-$0.812$\pm$0.041 & ... & ... & . & 1.591 & 0.32 & 0.38 & 2.11 & BLL & . & VLT & 55055\\
2FGL J1921.3$-$1231 & 290.349727 & $-$12.531772 & J1921$-$1231 & 1$\pm$0.12 & $-$0.631$\pm$0.271 & ... & ... & . & 1.190 & 0.77 & 0.96 & 1.76 & BLL & . & WMKO & 55476\\
2FGL J1921.9$-$1608 & 290.464844 & $-$16.120269 & J1921$-$1607 & 2.32$\pm$0.11 & $-$1.174$\pm$0.005 & ... & ... & . & ... & 0.30 & 0.30 & 1.64 & BLL & . & WMKO & 55061\\
2FGL J1927.0+6153 & 291.708132 & 61.911482 & J1926+6154 & 2.77$\pm$0.11 & $-$0.843$\pm$0.001 & ... & ... & . & ... & 0.23 & 0.24 & 1.65 & BLL & HBL & WMKO & 55060\\
2FGL J1927.5+6117 & 291.876906 & 61.292446 & J1927+6117 & 1.72$\pm$0.11 & $-$0.880$\pm$0.002 & ... & ... & . & ... & 0.31 & 0.34 & 1.92 & BLL & LBL & P200 & 53964\\
2FGL J1931.1+0938 & 292.788366 & 9.621420 & J1931+0937 & 2.47$\pm$0.11 & $-$0.484$\pm$0.027 & ... & ... & . & 0.476 & 0.20 & 0.23 & 1.85 & BLL & HBL & P200 & 55336\\
2FGL J1940.8$-$6213 & 295.340125 & $-$62.188889 & J1941$-$6211 & 0.43$\pm$0.12 & $-$1.971$\pm$0.125 & ... & ... & . & ... & 0.31 & 0.37 & 5.97 & UNK & . & NTT & 55776\\
2FGL J1946.1$-$3115 & 296.497648 & $-$31.194482 & J1945$-$3111 & 1.52$\pm$0.11 & $-$0.949$\pm$0.078 & ... & ... & . & ... & 0.53 & 0.53 & 1.97 & BLL & . & VLT & 55056\\
2FGL J2001.1+4352 & 300.304807 & 43.881390 & J2001+4352 & 2.96$\pm$0.11 & $-$0.952$\pm$0.005 & ... & ... & . & ... & 0.11 & 0.11 & 1.66 & BLL & IBL & WMKO & 55061\\
2FGL J2001.7+7042 & 300.391941 & 70.673681 & J2001+7040 & 0.88$\pm$0.23 & $-$1.195$\pm$2.374 & ... & ... & . & ... & 0.65 & 0.86 & 2.15 & BLL & LBL & WMKO & 55475\\
2FGL J2009.7+7225 & 302.468826 & 72.488705 & J2009+7229 & 1.32$\pm$0.11 & $-$1.474$\pm$0.006 & ... & ... & . & 1.740 & 0.64 & 0.66 & 2.03 & BLL & LBL & WMKO & 55357\\
2FGL J2012.1+4630 & 303.023274 & 46.482276 & J2012+4628 & 2.06$\pm$0.11 & $-$1.875$\pm$0.057 & ... & ... & . & ... & 0.19 & 0.27 & 2.12 & BLL & HBL & WMKO & 55357\\
2FGL J2014.0$-$0046 & 303.619188 & $-$0.790028 & J2014$-$0047 & 2.01$\pm$0.11 & $-$1.179$\pm$0.004 & $-$22.87$\pm$0.12 & 0.230 & G & ... & 0.23 & 0.23 & 1.63 & BLL & HBL & WMKO & 55061\\
2FGL J2015.1$-$0137 & 303.813103 & $-$1.625809 & J2015$-$0137 & 1.51$\pm$0.11 & $-$1.532$\pm$0.061 & ... & ... & . & ... & 0.47 & 0.57 & 1.78 & BLL & LBL & WMKO & 55358\\
2FGL J2015.6+3709 & 303.869729 & 37.183287 & J2015+3710 & 2.84$\pm$0.11 & $-$2.605$\pm$0.006 & ... & 0.859 & N & ... & 0.01 & 0.02 & 4.30 & FSRQ & LBL & WMKO & 55060\\
2FGL J2016.3$-$0904 & 304.100170 & $-$9.059201 & J2016$-$0903 & 2.1$\pm$0.11 & $-$0.419$\pm$0.004 & ... & ... & . & 0.605 & 0.67 & 0.67 & 1.63 & BLL & IBL & WMKO & 55476\\
2FGL J2022.3$-$4518 & 305.609458 & $-$45.225417 & J2022$-$4513 & 2.33$\pm$0.11 & $-$0.770$\pm$0.002 & ... & ... & . & ... & 0.28 & 0.28 & 1.96 & BLL & . & VLT & 55055\\
2FGL J2022.5+7614 & 305.647788 & 76.190666 & J2022+7611 & 1.8$\pm$0.13 & $-$1.707$\pm$0.224 & ... & 0.594 & G & ... & 0.39 & 0.41 & 1.68 & BLL & IBL & WMKO & 55061\\
2FGL J2023.4$-$1137 & 305.902923 & $-$11.666186 & J2023$-$1139 & -1.03$\pm$0.45 & $-$6.412$\pm$2.550 & ... & ... & . & ... & 0.73 & 0.89 & 5.14 & UNK & . & WMKO & 55040\\
2FGL J2025.1+3341 & 306.295148 & 33.716666 & J2025+3343 & 2.1$\pm$0.3 & 2.752$\pm$20.267 & ... & ... & . & ... & 0.01 & 0.01 & 7.05 & UNK & . & HET & 52601\\
2FGL J2029.4+4924 & 307.416140 & 49.439383 & J2029+4926 & 3.44$\pm$0.11 & $-$0.993$\pm$0.023 & ... & ... & . & ... & 0.03 & 0.03 & 2.38 & BLL & . & WMKO & 55060\\
2FGL J2036.6+6551 & 309.083224 & 65.887423 & J2036+6553 & 1.87$\pm$0.11 & $-$1.098$\pm$0.008 & ... & ... & . & ... & 0.30 & 0.42 & 1.71 & BLL & IBL & WMKO & 55061\\
2FGL J2039.1$-$1046 & 309.753069 & $-$10.778598 & J2039$-$1046 & 2.11$\pm$0.11 & $-$1.427$\pm$0.002 & ... & ... & . & ... & 0.34 & 0.41 & 1.63 & BLL & LBL & WMKO & 55061\\
2FGL J2042.1+2428 & 310.525376 & 24.447847 & J2042+2426 & 1.63$\pm$0.11 & $-$1.591$\pm$0.035 & $-$22.71$\pm$0.10 & 0.104 & G & ... & 0.10 & 0.10 & 1.78 & BLL & HBL & P200 & 55152\\
2FGL J2050.0+0408 & 312.526576 & 4.130620 & J2050+0407 & 2.08$\pm$0.11 & $-$1.665$\pm$0.021 & ... & ... & . & 1.271 & 0.25 & 0.37 & 1.64 & BLL & . & WMKO & 55060\\
2FGL J2055.4$-$0023 & 313.867623 & $-$0.354427 & J2055$-$0021 & 1.33$\pm$0.11 & $-$0.264$\pm$0.001 & $-$21.72$\pm$0.23 & 0.440 & G & ... & 0.44 & 0.44 & 1.63 & BLL & HBL & WMKO & 55476\\
2FGL J2108.7$-$0246 & 317.186258 & $-$2.842993 & J2108$-$0250 & 1.76$\pm$0.12 & $-$1.522$\pm$0.047 & $-$23.39$\pm$0.17 & 0.149 & G & ... & 0.15 & 0.15 & 2.68 & BLL & . & HET & 55478\\
2FGL J2116.2+3339 & 319.060594 & 33.655642 & J2116+3339 & 2.1$\pm$0.12 & $-$1.089$\pm$0.049 & ... & 1.596: & B & 0.766 & 0.24 & 0.58 & 1.63 & BLL & IBL & WMKO & 55475\\
2FGL J2127.8+3614 & 321.929352 & 36.218029 & J2127+3613 & 1.64$\pm$0.11 & $-$0.768$\pm$0.005 & ... & ... & . & 0.876 & 0.30 & 0.33 & 1.78 & BLL & IBL & P200 & 55064\\
2FGL J2139.3$-$4236 & 324.850792 & $-$42.588667 & J2139$-$4235 & 2.32$\pm$0.11 & $-$0.739$\pm$0.014 & ... & ... & . & ... & 0.50 & 0.54 & 1.91 & BLL & IBL & VLT & 55191\\
2FGL J2143.2$-$3929 & 325.761791 & $-$39.490004 & J2143$-$3929 & 1.31$\pm$0.11 & $-$0.729$\pm$0.017 & $-$22.51$\pm$0.11 & 0.429 & G & ... & 0.43 & 0.43 & 2.00 & BLL & . & VLT & 55191\\
2FGL J2146.6$-$1345 & 326.654200 & $-$13.733327 & J2146$-$1344 & 1.58$\pm$0.11 & $-$0.744$\pm$0.007 & ... & ... & . & ... & 0.71 & 0.74 & 1.64 & BLL & HBL & WMKO & 55358\\
2FGL J2149.6+0326 & 327.424626 & 3.380729 & J2149+0322 & 1.76$\pm$0.11 & $-$0.695$\pm$0.032 & ... & ... & . & 0.724 & 0.46 & 0.46 & 1.62 & BLL & . & WMKO & 55476\\
2FGL J2152.4+1735 & 328.103383 & 17.577241 & J2152+1734 & 1.43$\pm$0.11 & $-$1.423$\pm$0.003 & ... & 0.874 & B & ... & 0.56 & 0.59 & 1.80 & BLL & LBL & P200 & 55423\\
2FGL J2206.6$-$0029 & 331.680403 & $-$0.517331 & J2206$-$0031 & 1.09$\pm$0.11 & $-$1.005$\pm$0.009 & ... & 1.053 & B & ... & 0.76 & 0.93 & 1.78 & BLL & . & WMKO & 55476\\
2FGL J2206.6+6500 & 332.013806 & 65.327434 & J2208+6519 & 1.56$\pm$0.17 & $-$0.434$\pm$1.070 & ... & 1.121: & B & ... & 0.07 & 0.07 & 5.81 & FSRQ & . & HET & 52584\\
2FGL J2217.1+2422 & 334.253324 & 24.362696 & J2217+2421 & 1.6$\pm$0.12 & $-$1.457$\pm$0.118 & ... & ... & . & ... & 0.58 & 0.58 & 1.65 & BLL & LBL & WMKO & 55357\\
2FGL J2221.6$-$5223 & 335.372417 & $-$52.423750 & J2221$-$5225 & 1.76$\pm$0.11 & $-$0.738$\pm$0.024 & ... & ... & . & ... & 0.24 & 0.32 & 2.37 & BLL & HBL & NTT & 55207\\
2FGL J2223.4+0104 & 335.873229 & 1.040705 & J2223+0102 & 1.54$\pm$0.11 & $-$0.442$\pm$0.031 & ... & ... & . & ... & 0.68 & 0.81 & 1.63 & BLL & . & WMKO & 55476\\
2FGL J2236.1$-$3628 & 338.978417 & $-$36.484139 & J2235$-$3629 & 1.8$\pm$0.11 & $-$1.185$\pm$0.009 & ... & ... & . & ... & 0.30 & 0.38 & 2.23 & BLL & . & NTT & 55778\\
2FGL J2236.5$-$1431 & 339.142077 & $-$14.556198 & J2236$-$1433 & 2.56$\pm$0.11 & $-$1.526$\pm$0.001 & ... & ... & . & 0.608 & 0.14 & 0.20 & 2.53 & BLL & LBL & WMKO & 55358\\
2FGL J2236.4+2828 & 339.093599 & 28.482808 & J2236+2828 & 2.14$\pm$0.12 & $-$1.527$\pm$0.043 & ... & 0.790 & B & ... & 0.31 & 0.35 & 1.64 & BLL & LBL & HET & 55478\\
2FGL J2243.9+2021 & 340.978047 & 20.350953 & J2243+2021 & 2.54$\pm$0.11 & $-$0.922$\pm$0.001 & ... & ... & . & 0.395 & 0.28 & 0.35 & 1.64 & BLL & HBL & WMKO & 55061\\
2FGL J2247.2$-$0002 & 341.875756 & 0.001971 & J2247+0000 & 1.17$\pm$0.12 & $-$1.464$\pm$0.104 & ... & 0.949 & B & ... & 0.74 & 0.74 & 1.85 & BLL & IBL & WMKO & 55358\\
2FGL J2247.8+4412 & 341.971258 & 44.221353 & J2247+4413 & 1.74$\pm$0.12 & $-$0.694$\pm$0.052 & ... & ... & . & ... & 0.31 & 0.37 & 1.84 & BLL & HBL & P200 & 55567\\
2FGL J2251.9+4032 & 342.998908 & 40.515983 & J2251+4030 & 2.02$\pm$0.11 & $-$1.080$\pm$0.006 & $-$22.61$\pm$0.11 & 0.229 & G & ... & 0.23 & 0.23 & 1.67 & BLL & . & WMKO & 55357\\
2FGL J2255.2+2408 & 343.813936 & 24.170119 & J2255+2410 & 2.08$\pm$0.13 & $-$0.578$\pm$0.118 & ... & ... & . & ... & 0.32 & 0.47 & 2.49 & BLL & HBL & HET & 55415\\
2FGL J2256.4$-$2009 & 344.171622 & $-$20.194759 & J2256$-$2011 & 1.72$\pm$0.11 & $-$1.121$\pm$0.007 & ... & ... & . & ... & 0.56 & 0.72 & 1.93 & BLL & . & VLT & 55191\\
2FGL J2300.6+3139 & 345.095158 & 31.617882 & J2300+3137 & 1.41$\pm$0.11 & $-$1.198$\pm$0.332 & ... & ... & . & 1.498 & 0.41 & 0.52 & 2.10 & BLL & . & WMKO & 55039\\
2FGL J2304.7+3703 & 346.152632 & 37.085327 & J2304+3705 & 0.63$\pm$0.17 & $-$0.434$\pm$0.451 & ... & ... & . & ... & 0.47 & 0.47 & 3.25 & BLL & HBL & HET & 55390\\
2FGL J2308.0+1457 & 346.891839 & 14.838332 & J2307+1450 & 2.21$\pm$0.11 & $-$1.934$\pm$0.010 & ... & ... & . & ... & 0.29 & 0.29 & 1.66 & BLL & . & WMKO & 55060\\
2FGL J2310.9+0204 & 347.755415 & 2.085199 & J2311+0205 & 1.58$\pm$0.11 & $-$1.178$\pm$0.127 & ... & ... & . & ... & 0.38 & 0.57 & 1.76 & BLL & . & P200 & 55423\\
2FGL J2314.0+1446 & 348.488620 & 14.739600 & J2313+1444 & 1.68$\pm$0.14 & $-$1.696$\pm$0.168 & $-$23.66$\pm$0.17 & 0.164 & G & ... & 0.16 & 0.16 & 2.92 & BLL & HBL & HET & 52476\\
2FGL J2315.7$-$5014 & 348.934583 & $-$50.311028 & J2315$-$5018 & 1.27$\pm$0.11 & $-$1.176$\pm$0.114 & ... & 0.811 & B & ... & 0.54 & 0.61 & 2.03 & BLL & LBL & VLT & 55056\\
2FGL J2323.8+4212 & 350.967132 & 42.183465 & J2323+4210 & 1.81$\pm$0.12 & $-$0.838$\pm$0.028 & ... & ... & . & 0.268 & 0.49 & 0.64 & 1.70 & BLL & HBL & WMKO & 55357\\
2FGL J2325.3+3957 & 351.324428 & 39.960088 & J2325+3957 & 1.34$\pm$0.12 & $-$1.468$\pm$0.020 & ... & ... & . & 1.052 & 0.64 & 0.76 & 1.85 & BLL & LBL & WMKO & 55357\\
2FGL J2329.2+3755 & 352.309382 & 37.904105 & J2329+3754 & 1.73$\pm$0.11 & $-$0.765$\pm$0.074 & ... & ... & . & ... & 0.39 & 0.57 & 1.76 & BLL & HBL & P200 & 55424\\
2FGL J2334.8+1431 & 353.724434 & 14.537353 & J2334+1432 & 0.9$\pm$0.12 & $-$1.466$\pm$0.068 & ... & ... & . & ... & 0.41 & 0.45 & 2.66 & BLL & . & HET & 55390\\
2FGL J2352.0+1753 & 358.024445 & 17.820606 & J2352+1749 & 1.46$\pm$0.11 & $-$0.948$\pm$0.012 & ... & ... & . & 0.653 & 0.59 & 0.63 & 1.63 & BLL & . & WMKO & 55040\\
2FGL J2353.5$-$3034 & 358.447629 & $-$30.630123 & J2353$-$3037 & 1.15$\pm$0.11 & $-$1.255$\pm$0.008 & $-$22.91$\pm$0.26 & 0.737 & B & ... & 0.72 & 0.74 & 1.72 & BLL & . & WMKO & 55476\\

